The ALMA Survey of 70 $\mu \rm m$ Dark High-mass Clumps in Early Stages (ASHES). VII: Chemistry of Embedded Dense Cores

We present a study of chemistry toward 294 dense cores in 12 molecular clumps using the data obtained from the ALMA Survey of 70 $\mu \rm m$ dark High-mass clumps in Early Stages (ASHES). We identified 97 protostellar cores and 197 prestellar core candidates based on the detection of outflows and molecular transitions of high upper energy levels ($E_{u}/k > 45$ K). The detection rate of the N$_{2}$D$^{+}$ emission toward the protostellar cores is 38%, which is higher than 9% for the prestellar cores, indicating that N$_{2}$D$^{+}$ does not exclusively trace prestellar cores. The detection rates of the DCO$^{+}$ emission are 35% for the prestellar cores and 49% for the protostellar cores, which are higher than those of N$_{2}$D$^{+}$, implying that DCO$^{+}$ appears more frequently than N$_{2}$D$^{+}$ in both prestellar and protostellar cores. Both N$_{2}$D$^{+}$ and DCO$^{+}$ abundances appear to decrease from the prestellar to protostellar stage. The DCN, C$_{2}$D and $^{13}$CS emission lines are rarely seen in the dense cores of early evolutionary phases. The detection rate of the H$_{2}$CO emission toward dense cores is 52%, three times higher than that of CH$_{3}$OH (17%). In addition, the H$_{2}$CO detection rate, abundance, line intensities, and line widths increase with the core evolutionary status, suggesting that the H$_{2}$CO line emission is sensitive to protostellar activity.

==> apptab.tex <==

%--------------------------------------------------------------------------------------
\floattable
\begin{deluxetable*}{cccccccccccccccccccccccccccccccccccccccccc}
%\tabletypesize{\tiny}
\tabletypesize{\scriptsize}
\rotate
%\tablecolumns{9}
\tablewidth{0pc}
\tablecaption{Summary detected lines and their parameters. \label{tab:linepara}}
\tablehead{
\colhead{Molecule} & \colhead{core } & \colhead{$N_{\rm H_2}$} & \colhead{$n_{\rm H_2}$}& \colhead{$T_{\rm NH_3}$} & 
\colhead{$I_{\rm C^{18}O}$} & \colhead{$v_{\rm C^{18}O}$} & \colhead{$\sigma_{\rm C^{18}O}$} & \colhead{$N_{\rm C^{18}O}$} &  
\colhead{$I_{\rm DCO^{+}}$} & \colhead{$v_{\rm DCO^{+}}$} & \colhead{$\sigma_{\rm DCO^{+}}$} & \colhead{$N_{\rm DCO^{+}}$} & 
\colhead{$I_{\rm N_{2}D^{+}}$} & \colhead{$v_{\rm N_{2}D^{+}}$} & \colhead{$\sigma_{\rm N_{2}D^{+}}$} & \colhead{$N_{\rm N_{2}D^{+}}$} & 
\colhead{$I_{\rm H_{2}CO}$} & \colhead{$v_{\rm H_{2}CO}$} & \colhead{$\sigma_{\rm H_{2}CO}$} & \colhead{$N_{\rm H_{2}CO}$} & 
\colhead{$I_{\rm CH_{3}OH}$} & \colhead{$v_{\rm CH_{3}OH}$} & \colhead{$\sigma_{\rm CH_{3}OH}$} & \colhead{$N_{\rm CH_{3}OH}$} & 
\colhead{$I_{\rm SiO}$} & \colhead{$v_{\rm SiO}$} & \colhead{$\sigma_{\rm SiO}$} & \colhead{$N_{\rm SiO}$} & 
\colhead{$I_{\rm C_{2}D}$} & \colhead{$v_{\rm C_{2}D}$} & \colhead{$\sigma_{\rm C_{2}D}$} & \colhead{$N_{\rm C_{2}D}$} & 
\colhead{$I_{\rm DCN}$} & \colhead{$v_{\rm DCN}$} & \colhead{$\sigma_{\rm DCN}$} & \colhead{$N_{\rm DCN}$} & 
\colhead{$I_{\rm ^{13}CS}$} & \colhead{$v_{\rm ^{13}CS}$} & \colhead{$\sigma_{\rm ^{13}CS}$} & \colhead{$N_{\rm ^{13}CS}$} & 
\\
&  & \colhead{$\times 10^{22}$ cm$^{-2}$} & \colhead{$\times 10^{5}$ cm$^{-3}$} & \colhead{K} & 
\colhead{K} & \colhead{km s$^{-1}$} & \colhead{km s$^{-1}$} & \colhead{$\times 10^{14}$ cm$^{-2}$ } &
\colhead{K} & \colhead{km s$^{-1}$} & \colhead{km s$^{-1}$} & \colhead{$\times 10^{11}$ cm$^{-2}$ } &
\colhead{K} & \colhead{km s$^{-1}$} & \colhead{km s$^{-1}$} & \colhead{$\times 10^{11}$ cm$^{-2}$ } &
\colhead{K} & \colhead{km s$^{-1}$} & \colhead{km s$^{-1}$} & \colhead{$\times 10^{13}$ cm$^{-2}$ } &
\colhead{K} & \colhead{km s$^{-1}$} & \colhead{km s$^{-1}$} & \colhead{$\times 10^{13}$ cm$^{-2}$ } &
\colhead{K} & \colhead{km s$^{-1}$} & \colhead{km s$^{-1}$} & \colhead{$\times 10^{12}$ cm$^{-2}$ } &
\colhead{K} & \colhead{km s$^{-1}$} & \colhead{km s$^{-1}$} & \colhead{$\times 10^{12}$ cm$^{-2}$ } &
\colhead{K} & \colhead{km s$^{-1}$} & \colhead{km s$^{-1}$} & \colhead{$\times 10^{12}$ cm$^{-2}$ } &
\colhead{K} & \colhead{km s$^{-1}$} & \colhead{km s$^{-1}$} & \colhead{$\times 10^{12}$ cm$^{-2}$ } &
}
\startdata
G10.99 & 1 & 4.78  & 1.59  & 13.4 & 0.69 (0.09) & 30.16 (0.12) & 0.76 (0.12) & 8.35 (1.77) & 0.41 (0.03) & 29.75 (0.03) & 0.28 (0.03) & 1.92 (0.26) & 0.33 (0.03) & 29.69 (0.05) & 0.23 (0.12) & 2.34 (1.27) & 0.93 (0.01) & 30.21 (0.02) & 1.32 (0.02) & 1.25 (0.19) & 0.27 (0.01) & 30.04 (0.07) & 1.19 (0.07) & 1.36 (0.23) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G10.99 & 2 & 8.31  & 7.80  & 12.5 & 0.39 (0.08) & 29.96 (0.13) & 0.49 (0.11) & 3.21 (1.01) & - & - & - & - & 0.57 (0.06) & 29.89 (0.09) & 0.28 (0.25) & 4.84 (4.39) & 0.46 (0.04) & 28.67 (0.11) & 1.17 (0.11) & 0.55 (0.11) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G10.99 & 3 & 7.43  & 4.96  & 12.1 & 0.65 (0.04) & 29.92 (0.07) & 1.07 (0.07) & 11.69 (1.16) & 0.51 (0.05) & 29.63 (0.05) & 0.44 (0.05) & 4.02 (0.63) & 0.32 (0.03) & 29.97 (0.13) & 0.53 (0.38) & 4.64 (3.36) & 0.63 (0.02) & 30.28 (0.04) & 0.94 (0.04) & 0.61 (0.10) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G10.99 & 4 & 3.94  & 2.50  & 14.1 & - & - & - & - & - & - & - & - & 0.22 (0.02) & 30.01 (0.10) & 0.14 (0.07) & 2.66 (1.37) & 0.38 (0.02) & 29.89 (0.08) & 1.37 (0.08) & 0.53 (0.09) & 0.22 (0.02) & 29.72 (0.14) & 1.11 (0.14) & 0.95 (0.21) & 0.17 (0.02) & 28.13 (0.26) & 2.44 (0.26) & 1.77 (0.26) & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G10.99 & 5 & 7.63  & 3.21  & 10.8 & 0.62 (0.04) & 29.28 (0.09) & 1.12 (0.09) & 12.22 (1.47) & 0.79 (0.11) & 29.90 (0.03) & 0.18 (0.03) & 2.86 (0.62) & 0.71 (0.07) & 29.72 (0.06) & 0.22 (0.13) & 5.78 (3.60) & 0.17 (0.04) & 30.11 (0.17) & 0.64 (0.17) & 0.12 (0.05) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G10.99 & 6 & 5.45  & 5.41  & 13.2 & - & - & - & - & - & - & - & - & - & - & - & - & 1.06 (0.04) & 25.22 (0.22) & 4.69 (0.22) & 5.05 (0.81) & 1.21 (0.07) & 26.98 (0.16) & 2.36 (0.16) & 12.47 (2.16) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G10.99 & 7 & 5.36  & 2.18  & 12.2 & 1.23 (0.05) & 29.62 (0.04) & 0.85 (0.04) & 17.05 (1.36) & 1.74 (0.07) & 29.56 (0.01) & 0.19 (0.01) & 5.98 (0.49) & 0.55 (0.05) & 29.41 (0.04) & 0.18 (0.05) & 4.90 (1.38) & 0.20 (0.02) & 30.30 (0.14) & 1.07 (0.14) & 0.22 (0.05) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G10.99 & 8 & 4.85  & 1.57  & 12.3 & 0.80 (0.04) & 30.13 (0.04) & 0.70 (0.04) & 9.01 (0.87) & 0.44 (0.06) & 29.83 (0.05) & 0.30 (0.05) & 2.32 (0.52) & - & - & - & - & 0.22 (0.03) & 30.34 (0.11) & 0.71 (0.11) & 0.16 (0.04) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G10.99 & 9 & 5.29  & 3.03  & 11.5 & 0.84 (0.05) & 29.38 (0.05) & 0.74 (0.05) & 10.23 (0.99) & 0.66 (0.07) & 29.52 (0.04) & 0.35 (0.04) & 4.31 (0.72) & 0.56 (0.06) & 29.46 (0.07) & 0.20 (0.08) & 6.96 (2.89) & 0.23 (0.03) & 29.56 (0.17) & 1.27 (0.17) & 0.30 (0.07) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G10.99 & 10 & 2.90  & 1.33  & 12.8 & - & - & - & - & 0.29 (0.05) & 30.46 (0.05) & 0.28 (0.05) & 1.39 (0.36) & 0.42 (0.04) & 30.17 (0.05) & 0.11 (0.05) & 1.75 (0.84) & 0.38 (0.03) & 30.48 (0.07) & 0.68 (0.07) & 0.26 (0.05) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G10.99 & 11 & 5.27  & 5.84  & 11.8 & 0.33 (0.06) & 30.74 (0.23) & 1.10 (0.23) & 5.99 (1.68) & 0.87 (0.16) & 29.78 (0.03) & 0.13 (0.02) & 2.02 (0.55) & - & - & - & - & - & - & - & - & - & - & - & - & 1.09 (0.11) & 20.21 (0.05) & 0.34 (0.04) & 2.14 (0.34) & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G10.99 & 12 & 4.80  & 4.56  & 11.4 & 0.53 (0.09) & 30.14 (0.11) & 0.54 (0.11) & 4.74 (1.26) & - & - & - & - & - & - & - & - & 0.36 (0.04) & 31.83 (0.20) & 1.71 (0.20) & 0.64 (0.14) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G10.99 & 13 & 3.15  & 1.52  & 13.2 & 0.80 (0.06) & 28.99 (0.08) & 0.96 (0.08) & 11.83 (1.48) & - & - & - & - & - & - & - & - & 0.64 (0.03) & 29.05 (0.07) & 1.26 (0.07) & 0.82 (0.14) & 0.19 (0.03) & 28.82 (0.19) & 0.92 (0.19) & 0.78 (0.24) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G10.99 & 14 & 4.25  & 2.86  & 11.3 & 0.63 (0.07) & 29.50 (0.13) & 1.03 (0.13) & 10.60 (1.88) & 0.32 (0.06) & 28.76 (0.08) & 0.38 (0.08) & 2.32 (0.64) & - & - & - & - & 0.21 (0.03) & 29.89 (0.19) & 1.00 (0.19) & 0.22 (0.06) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G10.99 & 15 & 3.73  & 1.83  & 12.5 & 1.10 (0.09) & 29.54 (0.08) & 0.91 (0.08) & 15.76 (2.02) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G10.99 & 16 & 3.53  & 1.73  & 11.8 & 0.68 (0.07) & 27.84 (0.08) & 0.63 (0.08) & 6.79 (1.16) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G10.99 & 17 & 3.16  & 0.98  & 12.3 & 0.22 (0.05) & 28.97 (0.39) & 1.57 (0.39) & 5.49 (1.83) & 0.17 (0.03) & 29.31 (0.11) & 0.59 (0.11) & 1.75 (0.44) & - & - & - & - & 0.47 (0.02) & 30.62 (0.05) & 1.23 (0.05) & 0.60 (0.10) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G10.99 & 18 & 3.71  & 2.49  & 11.7 & 0.47 (0.07) & 27.91 (0.13) & 0.77 (0.13) & 5.83 (1.33) & 0.25 (0.06) & 28.86 (0.07) & 0.27 (0.07) & 1.24 (0.44) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G10.99 & 19 & 2.96  & 2.89  & 13.5 & 1.04 (0.10) & 29.76 (0.08) & 0.71 (0.08) & 11.27 (1.80) & - & - & - & - & - & - & - & - & 0.19 (0.05) & 30.12 (0.17) & 0.60 (0.17) & 0.12 (0.05) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G10.99 & 20 & 3.66  & 3.72  & 11.6 & 0.54 (0.10) & 29.53 (0.14) & 0.65 (0.14) & 5.59 (1.64) & 0.41 (0.07) & 28.55 (0.06) & 0.33 (0.06) & 2.58 (0.66) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G10.99 & 21 & 2.73  & 2.16  & 13.3 & 0.59 (0.08) & 29.63 (0.09) & 0.60 (0.10) & 5.35 (1.18) & 0.39 (0.05) & 29.65 (0.06) & 0.36 (0.06) & 2.35 (0.52) & - & - & - & - & 0.24 (0.04) & 29.65 (0.13) & 0.74 (0.13) & 0.18 (0.05) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G10.99 & 22 & 3.67  & 3.10  & 11.3 & 0.56 (0.07) & 28.03 (0.12) & 0.88 (0.12) & 7.96 (1.53) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G10.99 & 23 & 3.16  & 1.87  & 11.2 & 0.38 (0.05) & 28.47 (0.19) & 1.16 (0.19) & 7.12 (1.57) & - & - & - & - & - & - & - & - & 0.10 (0.02) & 29.22 (0.41) & 1.68 (0.41) & 0.18 (0.06) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G10.99 & 24 & 1.96  & 0.75  & 14.9 & 0.30 (0.07) & 29.18 (0.21) & 0.75 (0.21) & 3.34 (1.23) & - & - & - & - & - & - & - & - & 0.15 (0.02) & 30.38 (0.22) & 1.14 (0.22) & 0.17 (0.05) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G10.99 & 25 & 2.38  & 0.49  & 12.6 & 0.29 (0.05) & 28.63 (0.11) & 0.55 (0.10) & 2.44 (0.62) & 0.29 (0.05) & 28.89 (0.04) & 0.23 (0.04) & 1.14 (0.30) & - & - & - & - & 0.09 (0.01) & 30.08 (0.30) & 1.56 (0.30) & 0.14 (0.04) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G10.99 & 26 & 2.03  & 1.52  & 14.0 & - & - & - & - & - & - & - & - & - & - & - & - & 0.36 (0.03) & 29.20 (0.09) & 1.07 (0.09) & 0.39 (0.07) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G10.99 & 27 & 2.54  & 2.30  & 12.7 & 0.49 (0.08) & 29.84 (0.14) & 0.71 (0.14) & 5.29 (1.41) & 0.24 (0.05) & 29.80 (0.10) & 0.41 (0.10) & 1.71 (0.54) & 0.53 (0.05) & 29.44 (0.05) & 0.12 (0.08) & 2.69 (1.87) & 0.27 (0.03) & 30.43 (0.13) & 0.93 (0.13) & 0.26 (0.06) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G10.99 & 28 & 1.91  & 1.04  & 14.1 & 0.48 (0.08) & 27.67 (0.12) & 0.60 (0.12) & 4.29 (1.17) & - & - & - & - & - & - & - & - & 0.68 (0.02) & 28.85 (0.07) & 2.00 (0.07) & 1.37 (0.22) & 0.38 (0.03) & 28.49 (0.11) & 1.18 (0.11) & 1.74 (0.34) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G14.49 & 29 & 19.75  & 9.60  & 16.0 & 1.65 (0.06) & 40.06 (0.04) & 1.06 (0.04) & 34.21 (2.43) & 0.46 (0.03) & 38.82 (0.06) & 0.69 (0.06) & 4.86 (0.59) & 0.51 (0.05) & 38.55 (0.05) & 0.30 (0.08) & 5.82 (1.70) & 1.22 (0.03) & 40.33 (0.07) & 2.55 (0.07) & 3.18 (0.49) & 0.63 (0.02) & 39.51 (0.08) & 2.34 (0.08) & 4.69 (0.72) & 0.16 (0.01) & 30.07 (0.54) & 10.81 (0.54) & 6.68 (0.54) & - & - & - & - & 0.26 (0.02) & 39.35 (0.12) & 1.21 (0.12) & 1.64 (0.25) & - & - & - & - \\ 
G14.49 & 30 & 19.33  & 12.31  & 18.2 & 1.49 (0.03) & 39.96 (0.04) & 1.69 (0.04) & 51.72 (3.09) & - & - & - & - & - & - & - & - & 4.08 (0.07) & 41.71 (0.03) & 1.33 (0.03) & 5.75 (0.87) & 2.21 (0.05) & 41.19 (0.03) & 1.40 (0.03) & 8.38 (1.27) & 0.46 (0.02) & 40.18 (0.22) & 5.22 (0.22) & 8.08 (0.59) & - & - & - & - & 0.31 (0.03) & 41.25 (0.15) & 1.50 (0.15) & 2.05 (0.31) & - & - & - & - \\ 
G14.49 & 31 & 11.04  & 5.53  & 15.8 & 1.71 (0.06) & 40.69 (0.03) & 0.85 (0.03) & 25.01 (1.73) & - & - & - & - & 0.47 (0.05) & 41.05 (0.05) & 0.21 (0.08) & 2.73 (1.14) & 1.25 (0.05) & 41.23 (0.05) & 1.31 (0.05) & 1.67 (0.27) & 0.20 (0.01) & 39.17 (0.30) & 4.16 (0.30) & 2.74 (0.48) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G14.49 & 32 & 13.55  & 10.47  & 17.0 & 0.89 (0.04) & 41.09 (0.17) & 3.03 (0.17) & 49.02 (4.32) & - & - & - & - & - & - & - & - & 1.75 (0.03) & 39.86 (0.09) & 5.16 (0.09) & 9.34 (1.40) & 1.24 (0.04) & 38.90 (0.15) & 3.74 (0.15) & 13.63 (2.16) & 0.45 (0.01) & 42.67 (0.47) & 20.20 (0.52) & 32.39 (1.89) & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G14.49 & 33 & 13.43  & 12.49  & 16.5 & 2.46 (0.06) & 40.37 (0.03) & 1.09 (0.03) & 48.43 (2.89) & - & - & - & - & - & - & - & - & 1.15 (0.03) & 40.65 (0.03) & 0.96 (0.03) & 1.13 (0.17) & 0.78 (0.03) & 40.49 (0.04) & 0.76 (0.03) & 1.81 (0.29) & 0.47 (0.05) & 40.40 (0.07) & 0.54 (0.07) & 0.93 (0.16) & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G14.49 & 34 & 15.49  & 17.39  & 16.8 & 1.22 (0.04) & 39.36 (0.06) & 1.59 (0.06) & 36.13 (2.49) & 0.60 (0.11) & 39.29 (0.05) & 0.23 (0.05) & 2.06 (0.57) & 1.30 (0.13) & 41.39 (0.04) & 0.27 (0.09) & 10.67 (3.58) & 1.34 (0.05) & 44.18 (0.15) & 3.70 (0.15) & 5.10 (0.80) & 0.62 (0.06) & 41.39 (0.13) & 1.21 (0.13) & 2.21 (0.46) & 0.37 (0.02) & 48.89 (0.24) & 4.01 (0.24) & 5.30 (0.49) & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G14.49 & 35 & 11.72  & 6.58  & 16.1 & 2.11 (0.05) & 40.56 (0.02) & 0.97 (0.02) & 35.82 (2.11) & 0.64 (0.07) & 40.08 (0.03) & 0.22 (0.03) & 2.19 (0.38) & 1.83 (0.18) & 40.20 (0.02) & 0.21 (0.03) & 12.94 (2.22) & 0.54 (0.02) & 40.24 (0.05) & 0.90 (0.05) & 0.50 (0.08) & 0.26 (0.02) & 40.06 (0.10) & 1.16 (0.10) & 0.94 (0.18) & 0.37 (0.07) & 40.85 (0.05) & 0.25 (0.05) & 0.35 (0.10) & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G14.49 & 36 & 13.92  & 13.11  & 15.6 & 1.83 (0.07) & 40.19 (0.04) & 0.95 (0.04) & 31.39 (2.30) & 0.38 (0.06) & 40.66 (0.07) & 0.39 (0.07) & 2.33 (0.55) & 0.51 (0.05) & 40.35 (0.06) & 0.34 (0.18) & 4.27 (2.35) & 2.03 (0.05) & 40.78 (0.03) & 1.27 (0.03) & 2.63 (0.40) & 1.39 (0.03) & 40.29 (0.03) & 1.18 (0.03) & 5.42 (0.83) & 0.23 (0.01) & 39.14 (0.49) & 7.22 (0.49) & 6.56 (0.67) & - & - & - & - & 0.34 (0.07) & 40.26 (0.10) & 0.43 (0.10) & 0.77 (0.25) & - & - & - & - \\ 
G14.49 & 37 & 10.30  & 10.40  & 15.7 & 2.45 (0.05) & 41.10 (0.03) & 1.18 (0.03) & 48.98 (2.78) & - & - & - & - & 0.41 (0.04) & 40.27 (0.06) & 0.22 (0.11) & 2.54 (1.26) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G14.49 & 38 & 11.04  & 6.48  & 16.8 & 2.24 (0.05) & 40.35 (0.03) & 1.03 (0.03) & 40.27 (2.40) & - & - & - & - & 0.87 (0.09) & 40.27 (0.04) & 0.36 (0.13) & 7.58 (2.77) & 1.16 (0.02) & 41.23 (0.03) & 1.30 (0.03) & 1.55 (0.24) & 0.49 (0.02) & 40.70 (0.06) & 1.22 (0.06) & 1.76 (0.28) & 0.61 (0.05) & 40.76 (0.05) & 0.52 (0.05) & 1.14 (0.15) & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G14.49 & 39 & 13.48  & 8.29  & 14.6 & 1.55 (0.06) & 40.13 (0.04) & 1.00 (0.04) & 27.44 (2.07) & 0.29 (0.05) & 39.55 (0.13) & 0.66 (0.13) & 3.04 (0.78) & 1.34 (0.13) & 40.32 (0.03) & 0.29 (0.05) & 10.55 (2.01) & 0.39 (0.02) & 36.86 (0.20) & 4.26 (0.20) & 1.69 (0.27) & 0.22 (0.02) & 37.27 (0.31) & 3.71 (0.31) & 2.93 (0.54) & 0.18 (0.01) & 29.06 (0.52) & 8.48 (0.52) & 6.34 (0.60) & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G14.49 & 40 & 12.62  & 9.63  & 14.6 & 1.05 (0.05) & 40.18 (0.07) & 1.30 (0.07) & 23.77 (2.09) & 0.50 (0.07) & 38.72 (0.08) & 0.49 (0.08) & 3.82 (0.81) & 0.58 (0.06) & 38.48 (0.05) & 0.25 (0.13) & 3.99 (2.10) & 1.12 (0.03) & 41.26 (0.04) & 1.05 (0.04) & 1.20 (0.19) & 0.52 (0.04) & 41.09 (0.09) & 1.11 (0.09) & 2.08 (0.38) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G14.49 & 41 & 9.60  & 11.65  & 16.6 & 1.69 (0.07) & 39.84 (0.06) & 1.29 (0.06) & 36.96 (2.83) & 0.38 (0.07) & 39.78 (0.14) & 0.66 (0.14) & 3.76 (1.04) & - & - & - & - & 0.51 (0.02) & 41.26 (0.14) & 3.27 (0.14) & 1.73 (0.28) & 0.30 (0.02) & 40.64 (0.27) & 2.94 (0.27) & 2.64 (0.50) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G14.49 & 42 & 13.68  & 17.26  & 13.8 & 2.20 (0.06) & 40.31 (0.03) & 0.88 (0.03) & 34.04 (2.25) & 0.38 (0.06) & 40.44 (0.07) & 0.35 (0.07) & 2.17 (0.56) & 0.65 (0.06) & 40.19 (0.08) & 0.40 (0.18) & 6.68 (3.10) & 0.56 (0.02) & 34.62 (0.25) & 5.03 (0.25) & 2.84 (0.46) & 0.41 (0.03) & 35.56 (0.30) & 3.95 (0.30) & 6.53 (1.17) & 1.03 (0.03) & 31.78 (0.14) & 4.81 (0.14) & 22.20 (1.39) & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G14.49 & 43 & 12.15  & 17.25  & 14.4 & 1.12 (0.06) & 39.84 (0.07) & 1.13 (0.07) & 22.11 (2.04) & - & - & - & - & 0.40 (0.04) & 38.55 (0.06) & 0.18 (0.05) & 6.35 (1.78) & 0.67 (0.04) & 41.08 (0.06) & 0.85 (0.06) & 0.57 (0.10) & 0.16 (0.02) & 39.68 (0.38) & 2.19 (0.38) & 1.29 (0.35) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G14.49 & 44 & 10.01  & 4.17  & 13.9 & 1.19 (0.06) & 41.15 (0.10) & 1.78 (0.10) & 35.51 (3.08) & 0.31 (0.04) & 40.42 (0.05) & 0.38 (0.05) & 1.90 (0.35) & - & - & - & - & 0.26 (0.03) & 40.58 (0.07) & 0.60 (0.07) & 0.16 (0.03) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G14.49 & 45 & 9.83  & 6.15  & 13.6 & 1.70 (0.07) & 40.14 (0.04) & 0.83 (0.04) & 23.67 (1.95) & - & - & - & - & - & - & - & - & 0.27 (0.03) & 40.42 (0.12) & 1.00 (0.12) & 0.27 (0.06) & 0.22 (0.03) & 40.03 (0.13) & 0.79 (0.13) & 0.72 (0.19) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G14.49 & 46 & 8.29  & 3.61  & 14.9 & 0.66 (0.03) & 39.82 (0.10) & 1.94 (0.10) & 21.06 (1.81) & 0.32 (0.04) & 41.35 (0.05) & 0.35 (0.05) & 1.77 (0.36) & 0.62 (0.06) & 41.27 (0.04) & 0.15 (0.04) & 4.38 (1.38) & 1.39 (0.04) & 43.11 (0.19) & 6.04 (0.19) & 8.49 (1.31) & 0.59 (0.03) & 42.76 (0.37) & 6.98 (0.37) & 14.45 (2.37) & 0.62 (0.01) & 51.62 (0.27) & 11.07 (0.28) & 27.92 (1.64) & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G14.49 & 47 & 9.03  & 2.67  & 11.1 & 1.27 (0.05) & 44.33 (0.03) & 0.72 (0.03) & 15.78 (1.25) & - & - & - & - & 0.76 (0.08) & 38.14 (0.03) & 0.23 (0.06) & 7.03 (2.15) & 0.21 (0.01) & 40.72 (0.18) & 2.80 (0.18) & 0.64 (0.11) & 0.31 (0.02) & 39.43 (0.09) & 1.34 (0.09) & 2.66 (0.46) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G14.49 & 48 & 6.65  & 5.69  & 17.2 & 1.71 (0.07) & 40.42 (0.04) & 0.77 (0.04) & 21.40 (1.76) & 0.66 (0.09) & 37.67 (0.04) & 0.28 (0.04) & 2.73 (0.59) & - & - & - & - & 1.87 (0.06) & 41.01 (0.03) & 0.88 (0.03) & 1.71 (0.27) & 0.22 (0.02) & 35.97 (0.45) & 5.19 (0.45) & 3.34 (0.63) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G14.49 & 49 & 6.41  & 2.03  & 13.9 & 1.19 (0.04) & 40.73 (0.05) & 1.43 (0.05) & 27.07 (1.87) & 0.35 (0.07) & 40.07 (0.06) & 0.24 (0.06) & 1.35 (0.43) & 1.14 (0.11) & 39.70 (0.02) & 0.17 (0.04) & 6.10 (1.55) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G14.49 & 50 & 7.32  & 9.04  & 14.0 & 2.32 (0.07) & 39.96 (0.03) & 0.83 (0.03) & 31.08 (2.02) & - & - & - & - & - & - & - & - & 0.28 (0.03) & 40.65 (0.15) & 1.14 (0.15) & 0.33 (0.07) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G14.49 & 51 & 5.64  & 2.70  & 15.9 & 1.03 (0.08) & 44.32 (0.05) & 0.55 (0.05) & 8.91 (1.09) & - & - & - & - & - & - & - & - & 0.24 (0.02) & 37.86 (0.27) & 3.71 (0.27) & 0.91 (0.16) & - & - & - & - & 0.24 (0.03) & 35.58 (0.18) & 1.28 (0.18) & 1.16 (0.23) & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G14.49 & 52 & 5.38  & 5.49  & 16.2 & 1.40 (0.12) & 44.33 (0.06) & 0.62 (0.06) & 13.60 (1.88) & - & - & - & - & - & - & - & - & 0.61 (0.03) & 38.01 (0.10) & 1.85 (0.10) & 1.15 (0.19) & 0.36 (0.03) & 37.92 (0.14) & 1.63 (0.14) & 1.81 (0.34) & 0.45 (0.04) & 37.69 (0.10) & 1.09 (0.10) & 1.80 (0.24) & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G14.49 & 53 & 5.36  & 2.73  & 14.5 & 1.88 (0.04) & 40.83 (0.04) & 1.37 (0.04) & 40.23 (2.39) & - & - & - & - & - & - & - & - & - & - & - & - & 0.12 (0.02) & 38.28 (0.26) & 1.11 (0.26) & 0.48 (0.16) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G14.49 & 54 & 4.30  & 2.56  & 15.9 & 1.76 (0.06) & 44.09 (0.03) & 0.66 (0.03) & 17.89 (1.29) & - & - & - & - & - & - & - & - & 0.39 (0.03) & 38.58 (0.11) & 1.27 (0.11) & 0.51 (0.10) & 0.40 (0.03) & 38.68 (0.09) & 0.95 (0.09) & 1.21 (0.24) & 0.56 (0.05) & 38.97 (0.07) & 0.64 (0.07) & 1.36 (0.20) & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G14.49 & 55 & 5.52  & 3.51  & 14.7 & 2.39 (0.05) & 40.08 (0.02) & 0.90 (0.02) & 33.60 (1.98) & - & - & - & - & 0.61 (0.06) & 39.42 (0.04) & 0.13 (0.05) & 2.58 (0.94) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G14.49 & 56 & 3.94  & 1.75  & 15.2 & 0.89 (0.10) & 43.70 (0.07) & 0.55 (0.07) & 7.49 (1.29) & - & - & - & - & - & - & - & - & 0.38 (0.03) & 38.41 (0.16) & 1.87 (0.16) & 0.72 (0.13) & 0.47 (0.04) & 38.49 (0.07) & 0.79 (0.07) & 1.27 (0.24) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G14.49 & 57 & 4.94  & 3.55  & 14.8 & 1.96 (0.06) & 40.84 (0.05) & 1.29 (0.05) & 39.31 (2.68) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G14.49 & 58 & 4.36  & 3.96  & 15.2 & 1.38 (0.10) & 44.26 (0.05) & 0.55 (0.05) & 11.58 (1.42) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G14.49 & 59 & 3.90  & 1.32  & 15.6 & 1.07 (0.03) & 39.46 (0.03) & 1.06 (0.03) & 17.25 (1.12) & 0.31 (0.06) & 38.06 (0.05) & 0.25 (0.05) & 1.17 (0.33) & 0.46 (0.05) & 38.07 (0.03) & 0.14 (0.04) & 3.00 (0.83) & 0.35 (0.01) & 40.05 (0.08) & 1.63 (0.08) & 0.58 (0.09) & 0.17 (0.01) & 39.38 (0.19) & 1.86 (0.19) & 1.05 (0.21) & 0.15 (0.02) & 36.47 (0.17) & 1.23 (0.17) & 0.73 (0.14) & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G14.49 & 60 & 5.34  & 5.59  & 13.8 & 1.76 (0.07) & 42.10 (0.07) & 1.53 (0.07) & 42.37 (3.40) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G14.49 & 61 & 18.32  & 7.43  & 6.5 & 0.88 (0.08) & 44.12 (0.07) & 0.67 (0.07) & 17.98 (2.56) & - & - & - & - & - & - & - & - & 0.71 (0.03) & 39.96 (0.06) & 1.13 (0.06) & 1.56 (0.25) & 0.29 (0.03) & 39.47 (0.13) & 1.16 (0.13) & 19.01 (3.96) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G14.49 & 62 & 4.28  & 2.30  & 14.2 & 1.57 (0.06) & 41.59 (0.07) & 1.65 (0.07) & 39.70 (3.00) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G14.49 & 63 & 4.16  & 2.29  & 13.2 & 0.99 (0.08) & 43.37 (0.05) & 0.52 (0.05) & 8.00 (1.11) & - & - & - & - & 0.42 (0.04) & 40.57 (0.07) & 0.26 (0.19) & 3.15 (2.29) & 0.21 (0.03) & 41.17 (0.17) & 0.91 (0.17) & 0.19 (0.06) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G14.49 & 64 & 3.60  & 2.95  & 14.6 & 1.24 (0.06) & 41.58 (0.08) & 1.49 (0.08) & 27.85 (2.46) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G14.49 & 65 & 2.70  & 1.15  & 15.7 & 0.86 (0.05) & 38.67 (0.06) & 0.82 (0.06) & 10.47 (1.13) & - & - & - & - & - & - & - & - & 0.42 (0.03) & 39.91 (0.07) & 1.01 (0.07) & 0.43 (0.08) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G28.23 & 66 & 7.05  & 2.66  & 9.9 & 0.47 (0.03) & 79.03 (0.21) & 3.08 (0.21) & 26.23 (2.64) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G28.23 & 67 & 7.47  & 1.58  & 10.7 & 1.06 (0.03) & 79.95 (0.05) & 1.29 (0.05) & 23.66 (1.60) & 0.42 (0.04) & 79.97 (0.05) & 0.43 (0.05) & 3.55 (0.56) & 0.42 (0.04) & 79.94 (0.05) & 0.13 (0.04) & 5.35 (1.73) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G28.23 & 68 & 9.27  & 2.05  & 8.9 & 0.86 (0.03) & 80.77 (0.07) & 1.70 (0.07) & 28.98 (2.07) & 0.21 (0.03) & 80.88 (0.10) & 0.58 (0.10) & 3.02 (0.72) & - & - & - & - & 0.10 (0.01) & 80.88 (0.25) & 1.57 (0.25) & 0.19 (0.05) & 0.09 (0.02) & 71.67 (0.17) & 0.68 (0.17) & 0.84 (0.30) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G28.23 & 69 & 5.24  & 3.43  & 13.5 & 1.17 (0.06) & 79.91 (0.06) & 1.02 (0.06) & 18.70 (1.64) & 0.42 (0.08) & 79.70 (0.07) & 0.31 (0.07) & 2.11 (0.61) & - & - & - & - & 0.20 (0.03) & 79.35 (0.16) & 0.78 (0.16) & 0.16 (0.05) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G28.23 & 70 & 9.31  & 1.96  & 8.1 & 1.38 (0.04) & 79.25 (0.03) & 0.92 (0.03) & 27.33 (1.77) & 0.39 (0.04) & 79.32 (0.06) & 0.57 (0.06) & 6.50 (0.94) & - & - & - & - & 0.23 (0.02) & 79.19 (0.07) & 0.70 (0.07) & 0.22 (0.04) & 0.12 (0.02) & 79.14 (0.14) & 0.85 (0.14) & 1.99 (0.52) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G28.23 & 71 & 3.44  & 1.12  & 12.7 & 0.65 (0.06) & 80.81 (0.06) & 0.60 (0.06) & 6.04 (0.91) & 0.23 (0.04) & 80.05 (0.08) & 0.38 (0.08) & 1.48 (0.43) & - & - & - & - & 0.55 (0.02) & 82.10 (0.08) & 1.65 (0.08) & 0.93 (0.15) & 0.19 (0.02) & 82.03 (0.21) & 2.09 (0.21) & 1.90 (0.38) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G28.23 & 72 & 3.44  & 2.05  & 13.5 & 0.57 (0.09) & 78.90 (0.10) & 0.52 (0.09) & 4.49 (1.06) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G28.23 & 73 & 4.87  & 0.82  & 10.8 & 1.19 (0.04) & 78.93 (0.03) & 0.77 (0.03) & 15.23 (1.06) & 0.39 (0.03) & 78.74 (0.06) & 0.68 (0.06) & 5.21 (0.69) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G28.23 & 74 & 2.57  & 0.81  & 16.3 & 0.82 (0.10) & 73.69 (0.08) & 0.50 (0.07) & 6.12 (1.14) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G28.23 & 75 & 3.27  & 1.33  & 11.6 & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G28.23 & 76 & 3.15  & 0.68  & 11.5 & 0.35 (0.03) & 80.18 (0.19) & 1.76 (0.19) & 9.68 (1.43) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G28.23 & 77 & 4.04  & 0.75  & 9.5 & 0.33 (0.02) & 77.10 (0.21) & 3.43 (0.21) & 20.50 (1.94) & 0.44 (0.05) & 78.30 (0.04) & 0.32 (0.04) & 3.24 (0.57) & - & - & - & - & 0.12 (0.02) & 78.52 (0.17) & 0.91 (0.17) & 0.13 (0.04) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G28.23 & 78 & 5.87  & 1.45  & 7.0 & 0.51 (0.04) & 78.73 (0.12) & 1.20 (0.12) & 15.47 (2.15) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G327.11 & 79 & 6.82  & 2.56  & 14.1 & 0.23 (0.02) & -59.95 (0.11) & 1.44 (0.11) & 5.18 (0.59) & 0.22 (0.03) & -59.26 (0.05) & 0.32 (0.05) & 1.11 (0.22) & 0.33 (0.03) & -59.31 (0.04) & 0.19 (0.05) & 2.72 (0.78) & 0.60 (0.01) & -59.93 (0.05) & 1.97 (0.05) & 1.20 (0.18) & - & - & - & - & 0.06 (0.01) & -63.53 (1.04) & 7.87 (1.04) & 2.06 (0.37) & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G327.11 & 80 & 11.97  & 6.85  & 10.4 & 0.94 (0.05) & -55.02 (0.05) & 0.75 (0.05) & 12.71 (1.27) & 0.36 (0.07) & -59.37 (0.05) & 0.23 (0.05) & 1.71 (0.51) & 0.60 (0.06) & -59.33 (0.04) & 0.25 (0.12) & 5.68 (2.80) & 0.62 (0.02) & -58.49 (0.05) & 1.19 (0.05) & 0.81 (0.13) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G327.11 & 81 & 2.42  & 1.40  & 17.0 & 0.28 (0.04) & -57.30 (0.09) & 0.53 (0.10) & 2.14 (0.53) & - & - & - & - & 0.11 (0.01) & -58.92 (0.13) & 0.44 (0.35) & 1.23 (0.99) & 0.32 (0.01) & -57.98 (0.11) & 3.83 (0.11) & 1.28 (0.20) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G327.11 & 82 & 1.79  & 1.01  & 16.4 & 0.85 (0.03) & -57.94 (0.02) & 0.53 (0.03) & 6.50 (0.52) & - & - & - & - & 0.21 (0.02) & -59.48 (0.04) & 0.10 (0.04) & 0.70 (0.30) & 0.13 (0.01) & -59.31 (0.13) & 1.09 (0.13) & 0.14 (0.03) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G327.11 & 83 & 2.39  & 0.49  & 15.9 & 0.59 (0.03) & -59.29 (0.09) & 1.44 (0.09) & 12.37 (1.22) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G327.11 & 84 & 2.63  & 2.83  & 16.9 & 0.25 (0.02) & -59.05 (0.21) & 2.08 (0.21) & 7.70 (1.10) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G327.11 & 85 & 2.29  & 2.62  & 18.6 & 0.65 (0.03) & -60.23 (0.06) & 1.13 (0.06) & 10.83 (0.91) & 0.28 (0.05) & -59.20 (0.05) & 0.26 (0.05) & 1.05 (0.28) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G327.11 & 86 & 2.21  & 1.77  & 15.9 & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G327.11 & 87 & 2.32  & 0.84  & 14.6 & 0.95 (0.03) & -58.84 (0.02) & 0.76 (0.02) & 10.54 (0.67) & - & - & - & - & - & - & - & - & 0.07 (0.02) & -58.63 (0.15) & 0.58 (0.15) & 0.04 (0.02) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G327.11 & 88 & 2.77  & 0.95  & 12.6 & 0.21 (0.02) & -59.77 (0.13) & 1.47 (0.13) & 4.70 (0.59) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G327.11 & 89 & 3.21  & 0.90  & 11.1 & 0.27 (0.02) & -59.56 (0.11) & 1.47 (0.11) & 6.49 (0.69) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G327.11 & 90 & 1.31  & 0.76  & 20.4 & 0.52 (0.02) & -59.02 (0.08) & 1.66 (0.08) & 12.53 (1.03) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G327.11 & 91 & 1.78  & 0.23  & 15.9 & - & - & - & - & 0.19 (0.03) & -58.89 (0.07) & 0.38 (0.07) & 1.12 (0.28) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G327.11 & 92 & 1.77  & 0.82  & 14.7 & 1.47 (0.03) & -58.44 (0.02) & 0.67 (0.02) & 14.26 (0.82) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G327.11 & 93 & 2.16  & 1.88  & 13.4 & 1.11 (0.04) & -57.93 (0.03) & 0.59 (0.03) & 9.65 (0.74) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G327.11 & 94 & 1.84  & 1.40  & 14.2 & 0.57 (0.05) & -60.60 (0.05) & 0.55 (0.05) & 4.58 (0.62) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G327.11 & 95 & 1.40  & 0.86  & 15.9 & 0.48 (0.03) & -58.50 (0.11) & 1.30 (0.11) & 8.93 (1.06) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G327.11 & 96 & 0.81  & 0.80  & 22.5 & 0.79 (0.05) & -60.58 (0.04) & 0.63 (0.04) & 7.33 (0.74) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G327.11 & 97 & 0.91  & 0.44  & 18.3 & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G327.11 & 98 & 1.37  & 0.98  & 14.7 & 1.90 (0.04) & -58.20 (0.02) & 0.69 (0.02) & 18.97 (1.09) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G327.11 & 99 & 1.42  & 0.64  & 14.4 & 0.92 (0.03) & -58.72 (0.03) & 0.78 (0.03) & 10.35 (0.68) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G331.37 & 100 & 4.19  & 1.19  & 14.8 & 1.25 (0.06) & -87.54 (0.04) & 0.75 (0.04) & 14.18 (1.20) & 0.18 (0.03) & -87.72 (0.08) & 0.48 (0.08) & 1.38 (0.30) & 0.36 (0.04) & -87.71 (0.04) & 0.27 (0.06) & 2.69 (0.69) & 0.25 (0.01) & -88.33 (0.10) & 2.49 (0.10) & 0.64 (0.10) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G331.37 & 101 & 2.91  & 1.82  & 16.0 & 0.92 (0.10) & -88.00 (0.08) & 0.65 (0.08) & 8.83 (1.53) & - & - & - & - & - & - & - & - & 0.28 (0.02) & -87.87 (0.07) & 0.83 (0.07) & 0.24 (0.04) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G331.37 & 102 & 2.42  & 2.00  & 16.7 & 0.46 (0.09) & -89.68 (0.12) & 0.54 (0.11) & 3.59 (1.02) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G331.37 & 103 & 1.52  & 0.33  & 17.8 & 0.46 (0.13) & -88.70 (0.32) & 0.98 (0.32) & 6.48 (2.87) & - & - & - & - & - & - & - & - & 0.17 (0.01) & -89.67 (0.09) & 1.68 (0.09) & 0.31 (0.05) & - & - & - & - & 0.09 (0.01) & -90.80 (0.14) & 1.60 (0.14) & 0.51 (0.07) & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G331.37 & 104 & 1.82  & 0.84  & 17.9 & 0.88 (0.17) & -87.03 (0.14) & 0.61 (0.14) & 7.66 (2.33) & - & - & - & - & - & - & - & - & 0.17 (0.01) & -85.78 (0.18) & 2.01 (0.18) & 0.35 (0.07) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G331.37 & 105 & 2.07  & 0.91  & 16.0 & 1.19 (0.13) & -87.27 (0.08) & 0.63 (0.08) & 10.81 (1.92) & - & - & - & - & - & - & - & - & 0.15 (0.02) & -87.30 (0.13) & 1.02 (0.13) & 0.15 (0.03) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G331.37 & 106 & 2.10  & 0.68  & 16.0 & 1.77 (0.09) & -87.51 (0.03) & 0.44 (0.03) & 11.33 (1.06) & 0.40 (0.09) & -87.42 (0.07) & 0.27 (0.07) & 1.63 (0.57) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G331.37 & 107 & 3.28  & 0.78  & 12.3 & 2.73 (0.10) & -87.94 (0.03) & 0.60 (0.03) & 25.28 (1.93) & 0.64 (0.14) & -87.79 (0.03) & 0.12 (0.03) & 1.41 (0.49) & - & - & - & - & 0.30 (0.04) & -87.75 (0.10) & 0.64 (0.10) & 0.20 (0.05) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G331.37 & 108 & 3.28  & 2.82  & 12.9 & 0.98 (0.04) & -87.46 (0.04) & 0.76 (0.04) & 11.30 (0.93) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G331.37 & 109 & 2.09  & 1.16  & 16.0 & 1.32 (0.05) & -87.82 (0.02) & 0.41 (0.02) & 7.87 (0.57) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G331.37 & 110 & 4.97  & 2.90  & 9.0 & 1.13 (0.05) & -87.72 (0.03) & 0.39 (0.02) & 8.33 (0.71) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & 0.29 (0.07) & -102.25 (0.04) & 0.11 (0.03) & 8.91 (3.20) & - & - & - & - & - & - & - & - \\ 
G331.37 & 111 & 1.60  & 0.30  & 15.1 & - & - & - & - & 0.12 (0.02) & -88.15 (0.06) & 0.27 (0.06) & 0.51 (0.15) & 0.20 (0.02) & -88.19 (0.04) & 0.10 (0.03) & 1.12 (0.32) & 0.08 (0.01) & -88.48 (0.15) & 0.80 (0.15) & 0.06 (0.02) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G331.37 & 112 & 1.93  & 0.88  & 14.6 & - & - & - & - & 0.21 (0.05) & -88.23 (0.12) & 0.41 (0.12) & 1.39 (0.53) & - & - & - & - & 0.33 (0.04) & -87.95 (0.09) & 0.67 (0.09) & 0.23 (0.05) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G331.37 & 113 & 1.43  & 0.33  & 17.9 & 0.33 (0.04) & -87.05 (0.12) & 0.93 (0.12) & 4.45 (0.80) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G331.37 & 114 & 1.33  & 0.52  & 16.0 & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G331.37 & 115 & 1.66  & 0.86  & 16.0 & 0.61 (0.12) & -87.81 (0.11) & 0.39 (0.10) & 3.36 (1.09) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G331.37 & 116 & 1.60  & 0.93  & 16.0 & 0.81 (0.12) & -87.46 (0.11) & 0.64 (0.11) & 7.39 (1.77) & - & - & - & - & - & - & - & - & 0.14 (0.02) & -85.97 (0.27) & 1.82 (0.27) & 0.25 (0.06) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G331.37 & 117 & 1.73  & 1.30  & 16.0 & 1.20 (0.06) & -87.85 (0.03) & 0.53 (0.03) & 9.05 (0.78) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G331.37 & 118 & 1.33  & 1.27  & 18.1 & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & 0.27 (0.08) & -78.20 (0.15) & 0.46 (0.15) & 1.06 (0.46) \\ 
G331.37 & 119 & 1.14  & 0.55  & 17.0 & 0.66 (0.12) & -86.62 (0.09) & 0.49 (0.11) & 4.60 (1.38) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G331.37 & 120 & 1.18  & 0.75  & 16.0 & 0.52 (0.04) & -88.34 (0.06) & 0.61 (0.06) & 4.44 (0.62) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G331.37 & 121 & 1.38  & 0.48  & 17.1 & 1.02 (0.06) & -86.98 (0.05) & 0.68 (0.05) & 9.89 (1.02) & - & - & - & - & - & - & - & - & 0.19 (0.02) & -88.26 (0.07) & 0.69 (0.07) & 0.14 (0.03) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G331.37 & 122 & 1.50  & 0.87  & 16.0 & 1.12 (0.19) & -87.13 (0.12) & 0.62 (0.12) & 9.97 (2.57) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G331.37 & 123 & 1.14  & 0.40  & 18.1 & 0.61 (0.03) & -87.71 (0.07) & 1.05 (0.07) & 9.08 (0.89) & - & - & - & - & - & - & - & - & 0.24 (0.02) & -89.19 (0.08) & 0.98 (0.08) & 0.25 (0.04) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G331.37 & 124 & 1.19  & 0.56  & 16.0 & 0.83 (0.13) & -89.05 (0.10) & 0.39 (0.07) & 4.58 (1.07) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G331.37 & 125 & 1.25  & 0.47  & 17.8 & 0.38 (0.09) & -86.30 (0.27) & 0.94 (0.27) & 5.01 (1.91) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G331.37 & 126 & 1.49  & 0.79  & 16.0 & 1.06 (0.05) & -87.84 (0.03) & 0.53 (0.03) & 7.97 (0.68) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G331.37 & 127 & 1.24  & 0.44  & 17.5 & 0.42 (0.04) & -86.80 (0.12) & 1.04 (0.12) & 6.15 (0.97) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G331.37 & 128 & 1.23  & 0.67  & 17.9 & 0.83 (0.10) & -86.71 (0.10) & 0.71 (0.10) & 8.33 (1.55) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G331.37 & 129 & 1.30  & 1.05  & 18.0 & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G331.37 & 130 & 1.28  & 0.33  & 16.0 & 0.45 (0.04) & -88.20 (0.17) & 1.57 (0.17) & 9.96 (1.54) & - & - & - & - & - & - & - & - & 0.18 (0.03) & -88.94 (0.10) & 0.55 (0.10) & 0.10 (0.03) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G331.37 & 131 & 1.26  & 0.45  & 18.0 & 0.99 (0.19) & -87.32 (0.17) & 0.79 (0.17) & 11.06 (3.24) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G331.37 & 132 & 0.94  & 0.40  & 18.9 & 0.18 (0.05) & -87.93 (0.38) & 1.16 (0.38) & 3.01 (1.30) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G331.37 & 133 & 1.21  & 0.29  & 16.0 & 0.79 (0.04) & -87.61 (0.03) & 0.57 (0.03) & 6.34 (0.57) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G331.37 & 134 & 1.10  & 0.49  & 19.2 & 1.13 (0.16) & -87.27 (0.09) & 0.58 (0.09) & 9.33 (2.05) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G331.37 & 135 & 1.06  & 0.64  & 18.8 & 0.53 (0.13) & -87.52 (0.14) & 0.50 (0.14) & 3.80 (1.42) & 0.23 (0.05) & -88.32 (0.08) & 0.32 (0.08) & 1.07 (0.34) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G331.37 & 136 & 1.03  & 0.25  & 15.7 & 0.80 (0.12) & -88.41 (0.10) & 0.52 (0.09) & 5.95 (1.39) & - & - & - & - & - & - & - & - & 0.15 (0.02) & -88.77 (0.13) & 0.81 (0.13) & 0.12 (0.03) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G331.37 & 137 & 0.88  & 0.41  & 16.0 & 0.82 (0.05) & -88.29 (0.04) & 0.46 (0.03) & 5.38 (0.55) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G331.37 & 138 & 0.90  & 0.32  & 15.4 & 0.65 (0.05) & -89.12 (0.06) & 0.59 (0.05) & 5.42 (0.71) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G337.54 & 139 & 12.41  & 8.67  & 15.3 & 1.98 (0.06) & -53.79 (0.03) & 0.76 (0.03) & 26.43 (1.76) & 0.23 (0.02) & -54.62 (0.09) & 0.74 (0.09) & 2.58 (0.45) & - & - & - & - & 1.37 (0.01) & -54.27 (0.02) & 2.06 (0.02) & 2.88 (0.43) & 0.57 (0.01) & -54.59 (0.03) & 1.49 (0.03) & 2.85 (0.43) & 0.07 (0.01) & -54.80 (0.21) & 1.37 (0.21) & 0.38 (0.08) & - & - & - & - & 0.18 (0.01) & -54.63 (0.10) & 1.31 (0.10) & 1.30 (0.17) & 0.18 (0.02) & -55.05 (0.21) & 1.30 (0.21) & 1.89 (0.41) \\ 
G337.54 & 140 & 6.38  & 3.09  & 15.3 & 1.21 (0.07) & -54.16 (0.04) & 0.60 (0.04) & 11.65 (1.14) & 0.52 (0.04) & -54.72 (0.04) & 0.43 (0.04) & 3.46 (0.47) & 0.42 (0.04) & -54.79 (0.03) & 0.39 (0.11) & 3.94 (1.20) & 1.63 (0.01) & -52.81 (0.01) & 1.85 (0.01) & 3.07 (0.46) & 0.47 (0.01) & -52.92 (0.04) & 1.85 (0.04) & 2.93 (0.44) & - & - & - & - & - & - & - & - & 0.13 (0.01) & -54.24 (0.15) & 1.10 (0.15) & 0.76 (0.15) & - & - & - & - \\ 
G337.54 & 141 & 5.53  & 2.77  & 12.9 & 0.65 (0.04) & -55.83 (0.05) & 0.69 (0.05) & 7.20 (0.75) & 0.28 (0.03) & -54.42 (0.04) & 0.34 (0.04) & 1.58 (0.27) & 0.16 (0.02) & -54.50 (0.04) & 0.11 (0.03) & 1.25 (0.37) & 0.38 (0.01) & -54.34 (0.06) & 2.20 (0.06) & 0.85 (0.13) & 0.27 (0.01) & -54.90 (0.06) & 1.43 (0.06) & 1.75 (0.28) & 0.12 (0.01) & -55.22 (0.13) & 1.22 (0.13) & 0.70 (0.10) & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G337.54 & 142 & 3.10  & 1.84  & 15.2 & 0.23 (0.02) & -55.41 (0.13) & 1.53 (0.13) & 5.21 (0.65) & 0.56 (0.05) & -55.54 (0.02) & 0.16 (0.02) & 1.35 (0.20) & 0.21 (0.02) & -55.63 (0.04) & 0.15 (0.05) & 0.96 (0.31) & - & - & - & - & - & - & - & - & - & - & - & - & 0.22 (0.05) & -55.44 (0.04) & 0.13 (0.03) & 4.78 (1.61) & - & - & - & - & - & - & - & - \\ 
G337.54 & 143 & 4.76  & 3.87  & 11.0 & - & - & - & - & 0.35 (0.07) & -55.30 (0.05) & 0.20 (0.05) & 1.34 (0.42) & - & - & - & - & 0.12 (0.03) & -55.54 (0.11) & 0.50 (0.13) & 0.07 (0.02) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G337.54 & 144 & 3.10  & 0.69  & 13.3 & 1.13 (0.04) & -55.74 (0.03) & 0.75 (0.03) & 12.88 (0.99) & 0.19 (0.02) & -55.88 (0.03) & 0.20 (0.03) & 0.64 (0.13) & - & - & - & - & 0.18 (0.01) & -55.61 (0.06) & 0.86 (0.06) & 0.15 (0.03) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G337.54 & 145 & 2.62  & 1.47  & 12.4 & 0.48 (0.02) & -55.29 (0.10) & 1.78 (0.10) & 13.02 (1.14) & 0.14 (0.03) & -55.89 (0.05) & 0.19 (0.05) & 0.47 (0.16) & - & - & - & - & 0.16 (0.02) & -55.80 (0.08) & 0.72 (0.08) & 0.12 (0.02) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G337.54 & 146 & 3.53  & 1.76  & 13.1 & 0.92 (0.04) & -52.84 (0.04) & 0.85 (0.04) & 12.13 (0.99) & 0.40 (0.06) & -55.65 (0.03) & 0.17 (0.03) & 1.13 (0.27) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G337.54 & 147 & 3.03  & 1.06  & 12.9 & 0.99 (0.03) & -55.26 (0.03) & 0.93 (0.03) & 14.17 (0.97) & 0.44 (0.07) & -54.37 (0.06) & 0.33 (0.06) & 2.46 (0.59) & 0.15 (0.01) & -54.57 (0.08) & 0.40 (0.09) & 2.74 (0.70) & 0.31 (0.01) & -54.11 (0.05) & 1.10 (0.05) & 0.35 (0.05) & - & - & - & - & 0.14 (0.01) & -55.51 (0.17) & 2.49 (0.17) & 1.74 (0.18) & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G337.54 & 148 & 3.31  & 3.31  & 12.7 & 0.84 (0.05) & -56.07 (0.04) & 0.62 (0.04) & 7.99 (0.80) & 0.45 (0.07) & -56.09 (0.03) & 0.18 (0.03) & 1.42 (0.36) & - & - & - & - & 0.25 (0.02) & -55.86 (0.10) & 1.16 (0.10) & 0.29 (0.06) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G337.54 & 149 & 3.30  & 1.21  & 12.0 & 1.59 (0.04) & -55.36 (0.02) & 0.67 (0.02) & 16.66 (0.99) & 0.31 (0.05) & -55.77 (0.04) & 0.21 (0.04) & 1.18 (0.27) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G337.54 & 150 & 3.03  & 2.05  & 12.4 & 0.99 (0.04) & -55.03 (0.06) & 1.37 (0.06) & 21.07 (1.63) & 0.42 (0.05) & -55.89 (0.03) & 0.18 (0.03) & 1.30 (0.26) & - & - & - & - & 0.12 (0.02) & -55.72 (0.15) & 0.83 (0.15) & 0.10 (0.03) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G337.54 & 151 & 2.60  & 3.12  & 13.1 & 0.63 (0.04) & -56.07 (0.06) & 0.81 (0.06) & 7.73 (0.85) & - & - & - & - & - & - & - & - & 0.12 (0.01) & -55.90 (0.23) & 1.79 (0.23) & 0.23 (0.05) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & 0.30 (0.06) & -52.63 (0.07) & 0.31 (0.07) & 0.75 (0.23) \\ 
G337.54 & 152 & 1.70  & 0.57  & 15.1 & 0.65 (0.04) & -53.51 (0.12) & 1.91 (0.12) & 18.03 (1.75) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G337.54 & 153 & 1.39  & 0.91  & 16.6 & 1.13 (0.04) & -56.19 (0.04) & 0.83 (0.04) & 13.44 (1.02) & - & - & - & - & - & - & - & - & 0.36 (0.01) & -54.98 (0.08) & 2.27 (0.08) & 0.84 (0.13) & 0.12 (0.01) & -55.08 (0.20) & 2.12 (0.20) & 0.77 (0.15) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G337.54 & 154 & 2.49  & 2.85  & 12.5 & 1.02 (0.05) & -56.10 (0.04) & 0.72 (0.04) & 11.29 (1.07) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G337.54 & 155 & 1.17  & 0.19  & 15.2 & 0.94 (0.06) & -51.58 (0.04) & 0.59 (0.04) & 7.87 (0.84) & 0.22 (0.04) & -54.83 (0.05) & 0.24 (0.05) & 0.82 (0.23) & 0.14 (0.01) & -54.93 (0.05) & 0.14 (0.08) & 0.59 (0.35) & 0.70 (0.01) & -54.48 (0.02) & 1.58 (0.02) & 1.13 (0.17) & 0.26 (0.01) & -54.83 (0.05) & 1.39 (0.05) & 1.22 (0.19) & 0.14 (0.01) & -54.61 (0.13) & 3.01 (0.13) & 1.64 (0.12) & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G337.54 & 156 & 1.28  & 0.93  & 14.3 & 0.93 (0.05) & -54.18 (0.03) & 0.50 (0.03) & 6.70 (0.65) & - & - & - & - & - & - & - & - & 1.03 (0.01) & -53.64 (0.02) & 1.39 (0.02) & 1.45 (0.22) & 0.32 (0.01) & -53.65 (0.07) & 1.39 (0.07) & 1.65 (0.27) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G337.54 & 157 & 0.69  & 0.37  & 18.9 & 2.11 (0.05) & -52.14 (0.02) & 0.66 (0.02) & 19.82 (1.21) & - & - & - & - & - & - & - & - & 0.12 (0.01) & -54.63 (0.18) & 1.37 (0.18) & 0.17 (0.04) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G332.96 & 158 & 3.65  & 1.22  & 12.6 & 0.37 (0.03) & -68.35 (0.10) & 1.16 (0.10) & 6.56 (0.85) & 0.26 (0.03) & -67.61 (0.07) & 0.56 (0.07) & 2.56 (0.42) & 0.26 (0.03) & -67.65 (0.06) & 0.38 (0.09) & 2.71 (0.69) & 0.34 (0.02) & -67.54 (0.07) & 1.19 (0.07) & 0.42 (0.07) & 0.09 (0.02) & -68.39 (0.29) & 1.35 (0.29) & 0.59 (0.19) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G332.96 & 159 & 2.89  & 1.91  & 12.6 & 1.02 (0.09) & -67.52 (0.08) & 0.83 (0.08) & 12.94 (1.85) & 0.52 (0.08) & -67.04 (0.06) & 0.31 (0.06) & 2.85 (0.68) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G332.96 & 160 & 2.27  & 0.68  & 12.6 & 1.07 (0.05) & -67.05 (0.03) & 0.68 (0.03) & 11.05 (0.90) & - & - & - & - & - & - & - & - & 0.14 (0.02) & -66.42 (0.11) & 0.55 (0.10) & 0.08 (0.02) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G332.96 & 161 & 3.10  & 1.81  & 12.6 & 0.54 (0.04) & -66.63 (0.06) & 0.63 (0.06) & 5.21 (0.68) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G332.96 & 162 & 2.26  & 0.88  & 12.6 & 0.58 (0.04) & -66.90 (0.05) & 0.63 (0.05) & 5.56 (0.62) & 0.28 (0.04) & -66.64 (0.06) & 0.36 (0.06) & 1.72 (0.38) & - & - & - & - & 0.16 (0.02) & -66.42 (0.09) & 0.64 (0.09) & 0.11 (0.03) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G332.96 & 163 & 2.57  & 0.75  & 12.6 & 0.72 (0.04) & -67.08 (0.07) & 1.00 (0.07) & 11.00 (1.13) & 0.33 (0.03) & -66.76 (0.05) & 0.44 (0.05) & 2.55 (0.40) & 0.20 (0.02) & -66.58 (0.06) & 0.14 (0.04) & 2.07 (0.66) & 0.11 (0.02) & -66.46 (0.12) & 0.79 (0.12) & 0.09 (0.02) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G332.96 & 164 & 2.72  & 2.03  & 12.6 & 0.59 (0.05) & -66.43 (0.06) & 0.64 (0.06) & 5.80 (0.77) & 0.17 (0.03) & -66.81 (0.12) & 0.59 (0.12) & 1.77 (0.47) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & 0.22 (0.04) & -66.76 (0.06) & 0.27 (0.06) & 11.31 (3.54) & - & - & - & - & - & - & - & - \\ 
G332.96 & 165 & 2.07  & 1.34  & 12.6 & 0.36 (0.04) & -67.03 (0.10) & 0.69 (0.10) & 3.74 (0.73) & - & - & - & - & - & - & - & - & 0.11 (0.02) & -67.71 (0.18) & 0.88 (0.18) & 0.10 (0.03) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G332.96 & 166 & 1.91  & 0.76  & 12.6 & 0.47 (0.05) & -69.14 (0.07) & 0.63 (0.07) & 4.45 (0.73) & 0.26 (0.04) & -68.62 (0.07) & 0.42 (0.07) & 1.90 (0.44) & - & - & - & - & 0.13 (0.02) & -68.59 (0.19) & 1.06 (0.19) & 0.15 (0.04) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G332.96 & 167 & 2.06  & 1.89  & 12.6 & 0.77 (0.08) & -66.72 (0.06) & 0.53 (0.06) & 6.16 (0.96) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G332.96 & 168 & 1.89  & 0.69  & 12.6 & 0.93 (0.10) & -66.87 (0.06) & 0.53 (0.06) & 7.45 (1.25) & 0.22 (0.03) & -67.07 (0.06) & 0.40 (0.06) & 1.53 (0.31) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G332.96 & 169 & 1.63  & 1.14  & 12.6 & 0.42 (0.04) & -67.09 (0.08) & 0.74 (0.08) & 4.61 (0.66) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G332.96 & 170 & 1.86  & 1.36  & 12.6 & 0.66 (0.06) & -65.77 (0.06) & 0.59 (0.06) & 5.87 (0.89) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G332.96 & 171 & 1.82  & 1.37  & 12.6 & 0.79 (0.10) & -66.56 (0.11) & 0.76 (0.11) & 8.99 (1.84) & 0.19 (0.04) & -66.92 (0.08) & 0.39 (0.08) & 1.32 (0.38) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G332.96 & 172 & 1.63  & 1.01  & 12.6 & 0.76 (0.05) & -65.94 (0.05) & 0.67 (0.05) & 7.71 (0.89) & - & - & - & - & - & - & - & - & 0.20 (0.03) & -65.75 (0.10) & 0.42 (0.07) & 0.09 (0.02) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G332.96 & 173 & 1.58  & 1.03  & 12.6 & 0.84 (0.05) & -66.57 (0.04) & 0.61 (0.04) & 7.66 (0.74) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G332.96 & 174 & 1.38  & 0.94  & 12.6 & 0.90 (0.10) & -65.94 (0.11) & 0.90 (0.11) & 12.11 (2.03) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G332.96 & 175 & 1.78  & 0.80  & 12.6 & 0.87 (0.06) & -66.77 (0.04) & 0.54 (0.04) & 7.06 (0.79) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G332.96 & 176 & 1.50  & 1.03  & 12.6 & 0.56 (0.05) & -66.58 (0.11) & 0.98 (0.11) & 8.23 (1.26) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G332.96 & 177 & 1.32  & 0.56  & 12.6 & 0.67 (0.05) & -66.60 (0.08) & 0.91 (0.08) & 9.11 (1.18) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.17 & 178 & 2.10  & 1.19  & 17.7 & 0.98 (0.13) & -53.25 (0.10) & 0.68 (0.10) & 9.67 (1.95) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.17 & 179 & 1.77  & 0.59  & 16.7 & 0.88 (0.14) & -53.34 (0.07) & 0.48 (0.10) & 6.11 (1.60) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.17 & 180 & 0.89  & 0.24  & 19.1 & 1.96 (0.07) & -53.12 (0.02) & 0.57 (0.02) & 15.81 (1.15) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.17 & 181 & 1.11  & 0.24  & 18.0 & 0.33 (0.05) & -53.62 (0.10) & 0.55 (0.09) & 2.59 (0.58) & - & - & - & - & 0.14 (0.01) & -54.35 (0.14) & 0.42 (0.22) & 1.91 (1.01) & 0.17 (0.02) & -53.91 (0.11) & 0.90 (0.11) & 0.16 (0.03) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.17 & 182 & 1.44  & 1.04  & 15.6 & 1.18 (0.08) & -52.79 (0.07) & 1.01 (0.07) & 17.10 (1.86) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.17 & 183 & 1.39  & 0.48  & 14.1 & 0.18 (0.03) & -47.91 (0.27) & 1.50 (0.27) & 3.89 (0.94) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.17 & 184 & 0.96  & 0.27  & 17.7 & 0.32 (0.00) & -53.00 (0.00) & 1.32 (0.13) & 5.92 (0.66) & - & - & - & - & - & - & - & - & 0.16 (0.03) & -53.56 (0.12) & 0.52 (0.11) & 0.09 (0.03) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.17 & 185 & 0.81  & 0.16  & 18.2 & 1.73 (0.11) & -57.48 (0.06) & 0.80 (0.06) & 19.54 (2.18) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.17 & 186 & 1.03  & 0.46  & 16.7 & 1.29 (0.05) & -53.18 (0.04) & 0.75 (0.04) & 13.77 (1.09) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.17 & 187 & 0.98  & 0.36  & 16.1 & 0.42 (0.04) & -54.36 (0.10) & 0.96 (0.10) & 5.66 (0.85) & - & - & - & - & - & - & - & - & 0.24 (0.02) & -53.97 (0.10) & 0.98 (0.10) & 0.24 (0.05) & 0.15 (0.02) & -54.48 (0.16) & 0.99 (0.16) & 0.46 (0.12) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.17 & 188 & 0.95  & 0.45  & 17.9 & 0.91 (0.04) & -53.47 (0.14) & 2.93 (0.14) & 37.91 (3.00) & - & - & - & - & - & - & - & - & - & - & - & - & 0.10 (0.02) & -54.84 (0.21) & 0.90 (0.21) & 0.24 (0.08) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.17 & 189 & 0.85  & 0.59  & 18.0 & 0.67 (0.04) & -51.24 (0.13) & 1.91 (0.13) & 18.03 (1.80) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.17 & 190 & 0.79  & 0.14  & 17.7 & 0.52 (0.03) & -52.85 (0.10) & 1.33 (0.10) & 9.69 (1.08) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.17 & 191 & 0.68  & 0.27  & 19.3 & 1.66 (0.05) & -52.97 (0.02) & 0.64 (0.02) & 15.11 (1.03) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.17 & 192 & 0.69  & 0.28  & 17.7 & 1.83 (0.06) & -51.64 (0.03) & 0.86 (0.03) & 22.29 (1.53) & - & - & - & - & - & - & - & - & 0.22 (0.03) & -54.71 (0.08) & 0.54 (0.07) & 0.13 (0.03) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.17 & 193 & 0.50  & 0.17  & 20.9 & 1.06 (0.03) & -50.49 (0.05) & 1.57 (0.05) & 23.87 (1.52) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.22 & 194 & 4.14  & 0.71  & 14.6 & 0.93 (0.03) & -51.98 (0.10) & 2.39 (0.10) & 33.07 (2.49) & 0.49 (0.08) & -52.38 (0.05) & 0.26 (0.05) & 2.02 (0.51) & - & - & - & - & 0.27 (0.03) & -52.90 (0.11) & 0.84 (0.11) & 0.23 (0.05) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.22 & 195 & 3.43  & 1.25  & 15.4 & 1.00 (0.07) & -53.21 (0.07) & 0.83 (0.07) & 12.28 (1.51) & 0.19 (0.02) & -52.43 (0.04) & 0.29 (0.04) & 0.87 (0.15) & - & - & - & - & 0.12 (0.01) & -52.86 (0.08) & 0.70 (0.08) & 0.09 (0.02) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.22 & 196 & 2.90  & 1.53  & 14.6 & 1.92 (0.06) & -52.01 (0.05) & 1.20 (0.05) & 33.86 (2.39) & 0.44 (0.07) & -52.13 (0.06) & 0.33 (0.06) & 2.30 (0.56) & - & - & - & - & 0.34 (0.03) & -51.97 (0.09) & 0.88 (0.09) & 0.30 (0.06) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.22 & 197 & 3.19  & 0.50  & 14.6 & 1.66 (0.10) & -52.55 (0.04) & 0.57 (0.04) & 13.89 (1.41) & 0.45 (0.07) & -52.26 (0.07) & 0.41 (0.07) & 2.95 (0.68) & - & - & - & - & 0.22 (0.04) & -52.30 (0.10) & 0.44 (0.10) & 0.10 (0.03) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.22 & 198 & 2.36  & 1.10  & 16.1 & 1.70 (0.07) & -52.06 (0.07) & 1.33 (0.07) & 32.73 (2.70) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.22 & 199 & 1.79  & 2.22  & 14.6 & 1.53 (0.05) & -52.43 (0.04) & 1.12 (0.04) & 24.67 (1.72) & - & - & - & - & - & - & - & - & 0.13 (0.02) & -53.37 (0.08) & 0.56 (0.08) & 0.07 (0.02) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.22 & 200 & 1.97  & 1.18  & 14.6 & 0.42 (0.04) & -45.00 (0.20) & 1.63 (0.20) & 9.86 (1.68) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.22 & 201 & 2.55  & 0.78  & 13.6 & 2.09 (0.08) & -51.57 (0.04) & 0.87 (0.04) & 26.82 (2.06) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.22 & 202 & 2.56  & 1.06  & 11.7 & 2.40 (0.09) & -51.38 (0.03) & 0.68 (0.03) & 25.22 (1.85) & 0.24 (0.03) & -51.34 (0.05) & 0.31 (0.05) & 1.34 (0.30) & - & - & - & - & 0.14 (0.02) & -51.43 (0.10) & 0.48 (0.08) & 0.07 (0.02) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.22 & 203 & 2.27  & 0.87  & 15.1 & 1.44 (0.13) & -51.76 (0.07) & 0.68 (0.07) & 14.14 (2.04) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.22 & 204 & 2.32  & 0.45  & 14.5 & 1.72 (0.08) & -51.57 (0.05) & 0.80 (0.05) & 19.92 (1.78) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.22 & 205 & 1.85  & 0.51  & 16.3 & 0.77 (0.03) & -44.13 (0.08) & 2.02 (0.08) & 22.20 (1.62) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.22 & 206 & 1.27  & 0.97  & 18.3 & 2.02 (0.07) & -51.39 (0.03) & 0.92 (0.03) & 26.55 (1.84) & - & - & - & - & - & - & - & - & 0.11 (0.02) & -51.05 (0.21) & 1.34 (0.21) & 0.16 (0.04) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.22 & 207 & 1.58  & 0.37  & 14.6 & 2.25 (0.04) & -52.56 (0.03) & 1.14 (0.03) & 36.87 (2.10) & - & - & - & - & - & - & - & - & 0.11 (0.02) & -52.29 (0.28) & 1.44 (0.28) & 0.16 (0.05) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.22 & 208 & 1.73  & 0.35  & 14.6 & 1.64 (0.07) & -52.49 (0.03) & 0.63 (0.03) & 14.90 (1.22) & - & - & - & - & - & - & - & - & 0.15 (0.03) & -52.31 (0.16) & 0.76 (0.16) & 0.12 (0.04) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.22 & 209 & 1.73  & 0.99  & 14.4 & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.22 & 210 & 1.49  & 0.43  & 14.1 & 0.99 (0.08) & -52.76 (0.08) & 0.86 (0.08) & 12.20 (1.63) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.22 & 211 & 2.70  & 0.38  & 10.1 & 0.83 (0.03) & -51.86 (0.09) & 1.98 (0.09) & 27.45 (2.07) & 0.28 (0.04) & -52.04 (0.07) & 0.41 (0.07) & 2.46 (0.53) & - & - & - & - & 0.18 (0.02) & -52.38 (0.07) & 0.50 (0.08) & 0.10 (0.03) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.22 & 212 & 1.33  & 0.46  & 15.3 & 1.57 (0.07) & -46.84 (0.03) & 0.61 (0.03) & 13.78 (1.13) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.22 & 213 & 1.30  & 0.55  & 15.1 & 0.73 (0.04) & -44.01 (0.04) & 0.66 (0.04) & 6.94 (0.68) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.22 & 214 & 1.27  & 0.15  & 14.6 & 1.57 (0.06) & -50.89 (0.03) & 0.59 (0.03) & 13.30 (0.99) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.23 & 215 & 6.66  & 1.01  & 13.6 & 1.46 (0.03) & -49.55 (0.03) & 1.15 (0.03) & 26.22 (1.51) & - & - & - & - & 0.26 (0.03) & -50.46 (0.04) & 0.44 (0.08) & 2.92 (0.65) & 0.27 (0.01) & -50.93 (0.05) & 1.92 (0.05) & 0.53 (0.08) & 0.10 (0.01) & -51.31 (0.13) & 2.01 (0.13) & 0.80 (0.14) & 0.04 (0.00) & -52.56 (0.51) & 3.50 (0.51) & 0.63 (0.12) & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.23 & 216 & 4.60  & 1.26  & 15.4 & 2.18 (0.03) & -51.10 (0.02) & 1.31 (0.02) & 43.27 (2.31) & - & - & - & - & - & - & - & - & 0.34 (0.01) & -51.51 (0.09) & 1.92 (0.09) & 0.67 (0.11) & - & - & - & - & - & - & - & - & - & - & - & - & 0.26 (0.06) & -50.95 (0.05) & 0.19 (0.05) & 0.27 (0.09) & - & - & - & - \\ 
G340.23 & 217 & 4.86  & 4.11  & 15.3 & 1.81 (0.04) & -49.81 (0.04) & 1.36 (0.04) & 37.35 (2.29) & - & - & - & - & - & - & - & - & 0.61 (0.02) & -51.30 (0.07) & 1.72 (0.07) & 1.06 (0.17) & 0.10 (0.02) & -52.10 (0.42) & 2.17 (0.42) & 0.76 (0.22) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.23 & 218 & 3.51  & 1.98  & 15.2 & 4.73 (0.06) & -50.96 (0.01) & 0.79 (0.01) & 55.57 (2.89) & 0.74 (0.07) & -51.05 (0.04) & 0.36 (0.04) & 4.15 (0.65) & - & - & - & - & 0.41 (0.03) & -50.91 (0.07) & 0.74 (0.07) & 0.31 (0.06) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.23 & 219 & 3.55  & 0.75  & 14.9 & 1.29 (0.06) & -49.46 (0.03) & 0.65 (0.03) & 12.60 (1.05) & 0.25 (0.04) & -49.68 (0.07) & 0.38 (0.07) & 1.47 (0.35) & - & - & - & - & 0.17 (0.02) & -49.63 (0.09) & 0.71 (0.09) & 0.12 (0.03) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.23 & 220 & 2.93  & 2.05  & 16.6 & 3.31 (0.06) & -51.27 (0.02) & 0.94 (0.02) & 45.76 (2.60) & - & - & - & - & - & - & - & - & 0.44 (0.03) & -51.27 (0.07) & 0.78 (0.07) & 0.35 (0.07) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.23 & 221 & 2.68  & 0.63  & 15.8 & 2.19 (0.08) & -50.95 (0.04) & 0.98 (0.04) & 31.53 (2.35) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.23 & 222 & 2.01  & 1.25  & 14.1 & 1.26 (0.04) & -51.11 (0.04) & 1.30 (0.04) & 24.04 (1.56) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.23 & 223 & 2.98  & 1.20  & 15.5 & 1.30 (0.05) & -49.51 (0.03) & 0.83 (0.03) & 15.86 (1.15) & 0.19 (0.03) & -50.38 (0.09) & 0.51 (0.09) & 1.50 (0.35) & - & - & - & - & 0.15 (0.02) & -50.39 (0.16) & 1.02 (0.16) & 0.15 (0.04) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.23 & 224 & 2.49  & 1.15  & 14.6 & 1.22 (0.04) & -50.64 (0.05) & 1.42 (0.05) & 25.42 (1.70) & 0.28 (0.04) & -50.70 (0.05) & 0.35 (0.05) & 1.59 (0.33) & - & - & - & - & 0.17 (0.03) & -51.06 (0.08) & 0.50 (0.10) & 0.09 (0.03) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.23 & 225 & 1.94  & 1.17  & 17.2 & 2.84 (0.06) & -50.82 (0.02) & 1.02 (0.02) & 41.93 (2.38) & 0.24 (0.05) & -51.13 (0.08) & 0.34 (0.08) & 1.24 (0.38) & - & - & - & - & 0.36 (0.03) & -50.99 (0.07) & 0.65 (0.07) & 0.24 (0.05) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.23 & 226 & 2.06  & 1.21  & 16.0 & 0.69 (0.07) & -49.64 (0.06) & 0.49 (0.05) & 4.83 (0.71) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.23 & 227 & 1.42  & 0.51  & 18.7 & 1.10 (0.07) & -49.41 (0.04) & 0.61 (0.04) & 9.63 (1.01) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.23 & 228 & 1.93  & 0.83  & 16.2 & 0.87 (0.07) & -49.38 (0.08) & 0.85 (0.08) & 10.74 (1.39) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.23 & 229 & 1.53  & 1.10  & 15.8 & 1.52 (0.14) & -50.22 (0.07) & 0.67 (0.07) & 14.48 (2.14) & - & - & - & - & - & - & - & - & 0.35 (0.04) & -49.47 (0.08) & 0.62 (0.08) & 0.22 (0.05) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G340.23 & 230 & 1.34  & 0.81  & 15.8 & 0.34 (0.04) & -49.83 (0.32) & 2.49 (0.32) & 12.07 (2.10) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G341.03 & 231 & 9.87  & 5.47  & 9.3 & 1.84 (0.04) & -43.46 (0.02) & 0.85 (0.02) & 29.71 (1.73) & 0.43 (0.05) & -43.54 (0.04) & 0.29 (0.04) & 2.90 (0.54) & - & - & - & - & 0.59 (0.02) & -44.81 (0.08) & 2.37 (0.08) & 1.65 (0.26) & 0.18 (0.02) & -45.80 (0.22) & 2.16 (0.22) & 4.24 (0.85) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G341.03 & 232 & 6.26  & 3.91  & 11.5 & 0.62 (0.03) & -43.16 (0.04) & 0.83 (0.04) & 8.38 (0.66) & 0.85 (0.05) & -42.90 (0.01) & 0.19 (0.01) & 3.00 (0.29) & 0.33 (0.03) & -42.96 (0.04) & 0.15 (0.06) & 1.93 (0.86) & 0.26 (0.03) & -42.91 (0.05) & 0.40 (0.06) & 0.11 (0.03) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G341.03 & 233 & 5.07  & 3.42  & 14.4 & 2.87 (0.02) & -43.48 (0.01) & 0.91 (0.01) & 40.05 (2.01) & - & - & - & - & - & - & - & - & 0.42 (0.01) & -42.95 (0.04) & 0.91 (0.04) & 0.39 (0.06) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G341.03 & 234 & 4.65  & 1.52  & 11.0 & 1.64 (0.02) & -43.57 (0.02) & 0.92 (0.02) & 24.89 (1.33) & 0.26 (0.03) & -43.63 (0.04) & 0.27 (0.04) & 1.41 (0.28) & - & - & - & - & 0.31 (0.01) & -43.60 (0.05) & 0.85 (0.05) & 0.28 (0.05) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G341.03 & 235 & 6.07  & 2.25  & 11.4 & 1.28 (0.02) & -43.75 (0.02) & 0.85 (0.02) & 17.74 (0.98) & 0.24 (0.02) & -43.25 (0.03) & 0.31 (0.03) & 1.37 (0.21) & 0.20 (0.02) & -43.30 (0.05) & 0.24 (0.12) & 1.65 (0.84) & 0.12 (0.01) & -43.51 (0.06) & 0.58 (0.07) & 0.08 (0.02) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G341.03 & 236 & 3.65  & 0.91  & 13.4 & 1.44 (0.02) & -43.09 (0.01) & 0.70 (0.01) & 15.30 (0.80) & 0.40 (0.02) & -43.81 (0.02) & 0.26 (0.02) & 1.70 (0.16) & 0.15 (0.02) & -43.82 (0.04) & 0.15 (0.07) & 0.79 (0.39) & 0.19 (0.01) & -42.67 (0.04) & 0.89 (0.04) & 0.17 (0.03) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G341.03 & 237 & 5.26  & 5.48  & 13.9 & 2.84 (0.03) & -43.39 (0.01) & 0.86 (0.01) & 37.58 (1.93) & 0.55 (0.06) & -42.89 (0.02) & 0.18 (0.02) & 1.62 (0.27) & 0.21 (0.02) & -42.81 (0.08) & 0.25 (0.18) & 1.69 (1.22) & 0.36 (0.03) & -42.64 (0.04) & 0.48 (0.04) & 0.17 (0.03) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G341.03 & 238 & 4.26  & 5.15  & 14.6 & 3.12 (0.03) & -43.45 (0.01) & 0.77 (0.01) & 36.36 (1.84) & 0.28 (0.06) & -43.04 (0.05) & 0.19 (0.05) & 0.86 (0.27) & - & - & - & - & 0.34 (0.03) & -42.83 (0.03) & 0.45 (0.05) & 0.16 (0.03) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G341.03 & 239 & 3.41  & 2.05  & 12.8 & 1.22 (0.04) & -43.75 (0.04) & 1.07 (0.04) & 19.88 (1.31) & 0.31 (0.05) & -43.40 (0.03) & 0.17 (0.03) & 0.90 (0.21) & - & - & - & - & 0.31 (0.02) & -43.26 (0.03) & 0.50 (0.03) & 0.16 (0.03) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G341.03 & 240 & 1.66  & 1.25  & 20.8 & 2.47 (0.07) & -43.10 (0.02) & 0.57 (0.02) & 20.92 (1.41) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & 0.45 (0.08) & -42.13 (0.08) & 0.37 (0.08) & 1.53 (0.45) \\ 
G341.03 & 241 & 3.49  & 1.65  & 10.2 & 0.16 (0.03) & -43.29 (0.13) & 0.48 (0.10) & 1.29 (0.39) & 0.23 (0.05) & -43.00 (0.04) & 0.13 (0.03) & 0.63 (0.22) & - & - & - & - & 0.14 (0.02) & -43.08 (0.08) & 0.54 (0.08) & 0.08 (0.02) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G341.03 & 242 & 2.98  & 1.12  & 14.7 & 2.07 (0.03) & -43.17 (0.01) & 0.51 (0.01) & 15.59 (0.83) & 0.25 (0.02) & -43.43 (0.04) & 0.43 (0.04) & 1.71 (0.25) & - & - & - & - & 0.09 (0.01) & -43.03 (0.09) & 0.55 (0.09) & 0.05 (0.01) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G341.03 & 243 & 3.42  & 3.76  & 14.1 & 1.78 (0.03) & -44.02 (0.02) & 1.00 (0.02) & 26.52 (1.46) & - & - & - & - & - & - & - & - & 0.14 (0.02) & -43.37 (0.11) & 0.81 (0.11) & 0.11 (0.03) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G341.03 & 244 & 2.38  & 1.16  & 12.3 & 0.80 (0.02) & -42.72 (0.02) & 0.67 (0.02) & 8.15 (0.55) & 0.21 (0.03) & -42.51 (0.06) & 0.35 (0.06) & 1.29 (0.28) & 0.26 (0.03) & -42.45 (0.06) & 0.19 (0.07) & 2.63 (1.03) & 0.11 (0.01) & -42.67 (0.14) & 0.98 (0.14) & 0.11 (0.03) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G341.03 & 245 & 4.15  & 3.78  & 12.3 & 1.28 (0.03) & -44.00 (0.03) & 0.96 (0.03) & 19.23 (1.17) & 0.34 (0.07) & -43.06 (0.03) & 0.13 (0.04) & 0.80 (0.28) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G341.03 & 246 & 4.39  & 3.23  & 11.4 & 2.14 (0.03) & -43.36 (0.02) & 1.06 (0.02) & 36.48 (1.93) & 0.26 (0.04) & -43.57 (0.05) & 0.31 (0.05) & 1.51 (0.34) & 0.20 (0.02) & -43.60 (0.06) & 0.22 (0.14) & 1.64 (1.04) & 0.12 (0.02) & -43.70 (0.10) & 0.43 (0.08) & 0.05 (0.02) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G341.03 & 247 & 3.25  & 2.64  & 13.7 & 1.03 (0.03) & -42.82 (0.02) & 0.63 (0.02) & 9.66 (0.64) & - & - & - & - & - & - & - & - & 0.36 (0.02) & -42.43 (0.04) & 0.80 (0.04) & 0.29 (0.05) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G341.03 & 248 & 2.69  & 2.65  & 13.2 & 2.39 (0.10) & -43.52 (0.02) & 0.48 (0.02) & 17.25 (1.42) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G341.03 & 249 & 3.00  & 2.73  & 14.0 & 1.67 (0.03) & -42.43 (0.01) & 0.49 (0.01) & 12.17 (0.70) & 0.32 (0.05) & -42.52 (0.03) & 0.16 (0.03) & 0.86 (0.21) & - & - & - & - & 0.22 (0.04) & -42.30 (0.09) & 0.33 (0.07) & 0.07 (0.02) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G341.03 & 250 & 3.43  & 3.05  & 13.0 & 1.24 (0.04) & -44.14 (0.03) & 0.99 (0.03) & 18.64 (1.23) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G341.03 & 251 & 3.54  & 2.54  & 12.4 & 1.99 (0.04) & -43.41 (0.01) & 0.57 (0.01) & 17.51 (1.02) & 0.28 (0.04) & -43.24 (0.07) & 0.46 (0.07) & 2.27 (0.49) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G341.03 & 252 & 3.02  & 1.48  & 13.1 & 1.80 (0.03) & -43.38 (0.01) & 0.50 (0.01) & 13.65 (0.76) & 0.22 (0.03) & -43.40 (0.05) & 0.32 (0.05) & 1.20 (0.25) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G341.03 & 253 & 2.51  & 1.21  & 13.2 & 2.80 (0.07) & -43.51 (0.02) & 0.69 (0.02) & 28.66 (1.78) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G341.03 & 254 & 5.72  & 4.23  & 8.0 & 0.60 (0.03) & -44.26 (0.06) & 0.98 (0.06) & 12.46 (1.16) & 0.26 (0.03) & -42.94 (0.09) & 0.77 (0.09) & 6.10 (0.94) & - & - & - & - & 0.20 (0.03) & -42.87 (0.08) & 0.52 (0.09) & 0.14 (0.04) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G341.03 & 255 & 2.67  & 3.01  & 13.1 & 3.02 (0.04) & -43.64 (0.01) & 0.60 (0.01) & 27.21 (1.41) & 0.40 (0.05) & -43.49 (0.03) & 0.24 (0.03) & 1.63 (0.30) & - & - & - & - & 0.20 (0.04) & -43.58 (0.07) & 0.38 (0.09) & 0.08 (0.03) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G341.03 & 256 & 1.86  & 0.98  & 13.2 & 2.64 (0.05) & -43.25 (0.01) & 0.55 (0.01) & 21.34 (1.21) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G341.03 & 257 & 3.13  & 1.37  & 9.9 & 1.50 (0.04) & -43.28 (0.03) & 1.00 (0.03) & 25.92 (1.57) & 0.30 (0.05) & -43.45 (0.05) & 0.22 (0.05) & 1.47 (0.41) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G341.03 & 258 & 1.53  & 0.51  & 14.7 & 1.43 (0.04) & -43.92 (0.03) & 0.84 (0.03) & 17.26 (1.09) & 0.38 (0.07) & -43.16 (0.03) & 0.16 (0.03) & 0.95 (0.27) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G341.03 & 259 & 1.75  & 0.64  & 13.2 & 0.99 (0.04) & -43.51 (0.05) & 1.07 (0.05) & 15.55 (1.28) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G341.03 & 260 & 1.08  & 0.39  & 14.7 & 0.86 (0.02) & -43.41 (0.02) & 0.80 (0.02) & 9.77 (0.61) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G341.03 & 261 & 1.55  & 1.15  & 12.5 & 1.03 (0.07) & -45.20 (0.05) & 0.68 (0.05) & 10.54 (1.16) & 0.24 (0.06) & -42.89 (0.03) & 0.13 (0.04) & 0.53 (0.20) & - & - & - & - & 0.09 (0.01) & -46.14 (0.18) & 1.01 (0.18) & 0.09 (0.03) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G341.03 & 262 & 1.49  & 1.14  & 12.3 & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G341.03 & 263 & 1.45  & 0.87  & 13.1 & 0.80 (0.03) & -43.68 (0.07) & 1.75 (0.07) & 20.65 (1.51) & - & - & - & - & - & - & - & - & 0.07 (0.01) & -44.76 (0.33) & 2.03 (0.33) & 0.13 (0.04) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G341.03 & 264 & 1.08  & 0.80  & 14.8 & 1.58 (0.03) & -43.00 (0.02) & 0.95 (0.02) & 21.37 (1.26) & 0.34 (0.04) & -42.56 (0.04) & 0.25 (0.04) & 1.34 (0.27) & - & - & - & - & 0.24 (0.02) & -42.33 (0.05) & 0.54 (0.05) & 0.13 (0.03) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G341.03 & 265 & 1.08  & 0.43  & 13.2 & 0.78 (0.04) & -42.32 (0.02) & 0.45 (0.03) & 5.17 (0.53) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G343.48 & 266 & 7.67  & 6.60  & 16.1 & 0.77 (0.02) & -28.79 (0.02) & 0.89 (0.02) & 11.72 (0.67) & 0.44 (0.02) & -28.85 (0.02) & 0.36 (0.02) & 2.41 (0.19) & 0.23 (0.02) & -28.79 (0.04) & 0.18 (0.05) & 1.70 (0.49) & 1.55 (0.02) & -28.69 (0.03) & 1.82 (0.03) & 2.88 (0.43) & 0.65 (0.02) & -28.73 (0.05) & 1.76 (0.05) & 3.58 (0.55) & 0.21 (0.01) & -28.90 (0.16) & 4.07 (0.16) & 3.20 (0.23) & - & - & - & - & 0.07 (0.01) & -29.24 (0.16) & 1.54 (0.16) & 0.55 (0.08) & - & - & - & - \\ 
G343.48 & 267 & 4.74  & 5.12  & 15.3 & 0.84 (0.04) & -29.17 (0.04) & 0.82 (0.04) & 11.12 (0.95) & 0.35 (0.07) & -28.74 (0.02) & 0.12 (0.03) & 0.62 (0.20) & - & - & - & - & 0.85 (0.01) & -29.93 (0.02) & 1.19 (0.02) & 1.03 (0.15) & 0.30 (0.01) & -29.76 (0.06) & 1.13 (0.06) & 1.13 (0.19) & 0.11 (0.02) & -28.77 (0.10) & 0.53 (0.10) & 0.23 (0.06) & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G343.48 & 268 & 4.42  & 3.39  & 12.1 & 0.28 (0.02) & -28.42 (0.05) & 0.56 (0.05) & 2.55 (0.33) & 0.32 (0.04) & -28.40 (0.03) & 0.20 (0.03) & 1.15 (0.21) & 0.22 (0.02) & -28.47 (0.06) & 0.32 (0.17) & 2.17 (1.15) & 0.26 (0.01) & -28.22 (0.05) & 0.94 (0.05) & 0.25 (0.04) & - & - & - & - & 0.10 (0.01) & -28.72 (0.15) & 0.94 (0.15) & 0.49 (0.10) & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G343.48 & 269 & 2.38  & 1.87  & 12.0 & - & - & - & - & 0.11 (0.02) & -28.39 (0.09) & 0.59 (0.09) & 1.21 (0.26) & 0.23 (0.02) & -28.25 (0.06) & 0.22 (0.08) & 2.63 (1.05) & 0.15 (0.01) & -28.77 (0.07) & 0.69 (0.07) & 0.11 (0.02) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G343.48 & 270 & 3.44  & 4.34  & 9.9 & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G343.48 & 271 & 2.70  & 2.30  & 12.5 & 0.47 (0.03) & -28.71 (0.04) & 0.49 (0.03) & 3.57 (0.37) & 0.77 (0.04) & -28.59 (0.01) & 0.23 (0.01) & 3.08 (0.29) & 0.52 (0.05) & -28.62 (0.03) & 0.19 (0.06) & 3.55 (1.09) & 0.33 (0.02) & -28.52 (0.04) & 0.61 (0.03) & 0.21 (0.03) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G343.48 & 272 & 2.29  & 3.23  & 11.8 & - & - & - & - & - & - & - & - & - & - & - & - & 0.30 (0.02) & -28.58 (0.09) & 0.92 (0.09) & 0.29 (0.06) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G343.48 & 273 & 3.21  & 1.61  & 10.7 & 0.82 (0.02) & -28.47 (0.02) & 0.64 (0.02) & 8.78 (0.58) & 0.94 (0.04) & -28.46 (0.01) & 0.22 (0.01) & 4.08 (0.36) & 0.55 (0.05) & -28.57 (0.02) & 0.15 (0.03) & 4.78 (1.04) & 0.19 (0.02) & -28.44 (0.06) & 0.47 (0.04) & 0.10 (0.02) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G343.48 & 274 & 1.68  & 2.73  & 17.5 & 0.59 (0.03) & -28.60 (0.08) & 1.27 (0.08) & 11.09 (1.07) & 0.52 (0.05) & -29.04 (0.03) & 0.25 (0.03) & 1.90 (0.29) & - & - & - & - & 0.51 (0.02) & -29.95 (0.04) & 1.16 (0.04) & 0.62 (0.10) & 0.18 (0.02) & -29.88 (0.09) & 0.83 (0.09) & 0.42 (0.09) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G343.48 & 275 & 1.19  & 1.61  & 19.6 & 0.86 (0.03) & -28.70 (0.03) & 0.61 (0.03) & 7.72 (0.59) & 0.65 (0.04) & -28.42 (0.02) & 0.30 (0.02) & 2.88 (0.31) & - & - & - & - & 0.64 (0.01) & -27.32 (0.03) & 1.46 (0.03) & 1.01 (0.15) & 0.29 (0.01) & -27.10 (0.07) & 1.24 (0.07) & 0.91 (0.15) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G343.48 & 276 & 1.46  & 2.19  & 13.5 & 0.36 (0.03) & -28.11 (0.08) & 0.68 (0.07) & 3.63 (0.56) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G343.48 & 277 & 2.96  & 1.66  & 9.0 & 0.22 (0.04) & -27.72 (0.08) & 0.50 (0.10) & 2.06 (0.56) & 0.19 (0.02) & -28.68 (0.08) & 0.57 (0.08) & 2.79 (0.56) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G343.48 & 278 & 1.95  & 1.91  & 11.8 & 0.70 (0.07) & -28.35 (0.04) & 0.48 (0.06) & 5.24 (0.87) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G343.48 & 279 & 4.38  & 3.90  & 7.6 & - & - & - & - & 0.58 (0.09) & -28.37 (0.04) & 0.19 (0.04) & 3.76 (0.95) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G343.48 & 280 & 3.68  & 3.16  & 8.2 & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G343.48 & 281 & 1.72  & 1.27  & 11.8 & 0.88 (0.04) & -28.19 (0.03) & 0.62 (0.03) & 8.59 (0.70) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G343.48 & 282 & 1.08  & 0.82  & 14.8 & - & - & - & - & 0.36 (0.05) & -28.94 (0.03) & 0.21 (0.03) & 1.21 (0.26) & - & - & - & - & 0.10 (0.01) & -26.56 (0.22) & 1.50 (0.22) & 0.15 (0.04) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G343.48 & 283 & 1.61  & 0.54  & 11.8 & - & - & - & - & 0.27 (0.06) & -28.51 (0.04) & 0.12 (0.03) & 0.57 (0.21) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G343.48 & 284 & 1.50  & 1.15  & 12.1 & - & - & - & - & - & - & - & - & - & - & - & - & 0.20 (0.01) & -27.17 (0.14) & 3.09 (0.14) & 0.63 (0.10) & 0.10 (0.01) & -27.00 (0.27) & 2.83 (0.27) & 1.47 (0.29) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G343.48 & 285 & 2.02  & 1.67  & 10.0 & 0.43 (0.04) & -28.17 (0.05) & 0.49 (0.05) & 3.63 (0.55) & 0.47 (0.06) & -28.20 (0.03) & 0.18 (0.03) & 1.80 (0.38) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G343.48 & 286 & 2.37  & 1.56  & 8.8 & 0.68 (0.03) & -28.11 (0.03) & 0.63 (0.03) & 8.14 (0.70) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G343.48 & 287 & 1.20  & 0.60  & 13.3 & - & - & - & - & 0.37 (0.09) & -28.76 (0.02) & 0.10 (0.03) & 0.61 (0.23) & - & - & - & - & 0.12 (0.01) & -25.03 (0.11) & 0.94 (0.11) & 0.12 (0.03) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G343.48 & 288 & 1.04  & 1.33  & 13.1 & - & - & - & - & 0.38 (0.06) & -28.62 (0.02) & 0.13 (0.02) & 0.85 (0.19) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G343.48 & 289 & 1.43  & 0.57  & 11.4 & - & - & - & - & 0.23 (0.04) & -28.93 (0.04) & 0.19 (0.04) & 0.83 (0.24) & 0.17 (0.02) & -28.89 (0.07) & 0.22 (0.15) & 1.32 (0.91) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G343.48 & 290 & 0.86  & 0.49  & 14.8 & 0.18 (0.02) & -28.25 (0.15) & 0.92 (0.15) & 2.33 (0.51) & - & - & - & - & - & - & - & - & 0.32 (0.01) & -26.38 (0.06) & 1.43 (0.06) & 0.47 (0.07) & 0.20 (0.01) & -26.22 (0.09) & 1.16 (0.09) & 0.82 (0.15) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G343.48 & 291 & 0.48  & 0.55  & 22.8 & 1.00 (0.03) & -28.84 (0.02) & 0.60 (0.02) & 8.88 (0.63) & - & - & - & - & - & - & - & - & 0.13 (0.02) & -29.55 (0.11) & 0.56 (0.11) & 0.09 (0.03) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G343.48 & 292 & 0.88  & 0.70  & 14.2 & 0.46 (0.03) & -28.73 (0.04) & 0.40 (0.02) & 2.67 (0.26) & - & - & - & - & - & - & - & - & 0.07 (0.01) & -28.57 (0.37) & 2.13 (0.37) & 0.14 (0.04) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G343.48 & 293 & 0.78  & 0.62  & 16.2 & 0.81 (0.03) & -28.40 (0.02) & 0.52 (0.02) & 6.06 (0.47) & 0.33 (0.05) & -28.38 (0.03) & 0.16 (0.03) & 0.80 (0.20) & - & - & - & - & 0.36 (0.01) & -27.18 (0.05) & 1.40 (0.05) & 0.51 (0.08) & 0.10 (0.01) & -27.44 (0.20) & 1.23 (0.20) & 0.38 (0.10) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
G343.48 & 294 & 1.05  & 0.62  & 12.0 & 0.11 (0.02) & -26.20 (0.17) & 0.88 (0.17) & 1.52 (0.40) & - & - & - & - & - & - & - & - & 0.14 (0.01) & -27.18 (0.13) & 1.78 (0.13) & 0.27 (0.05) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
\enddata
\tablenotetext{}{Notes. 
}
\end{deluxetable*}
%--------------------------------------------------------------------------------------





